Distributed Energy Management and Demand Response in Smart Grids: A Multi-Agent Deep Reinforcement Learning Framework

This paper presents a multi-agent Deep Reinforcement Learning (DRL) framework for autonomous control and integration of renewable energy resources into smart power grid systems. In particular, the proposed framework jointly considers demand response (DR) and distributed energy management (DEM) for residential end-users. DR has a widely recognized potential for improving power grid stability and reliability, while at the same time reducing end-users energy bills. However, the conventional DR techniques come with several shortcomings, such as the inability to handle operational uncertainties while incurring end-user disutility, which prevents widespread adoption in real-world applications. The proposed framework addresses these shortcomings by implementing DR and DEM based on real-time pricing strategy that is achieved using deep reinforcement learning. Furthermore, this framework enables the power grid service provider to leverage distributed energy resources (i.e., PV rooftop panels and battery storage) as dispatchable assets to support the smart grid during peak hours, thus achieving management of distributed energy resources. Simulation results based on the Deep Q-Network (DQN) demonstrate significant improvements of the 24-hour accumulative profit for both prosumers and the power grid service provider, as well as major reductions in the utilization of the power grid reserve generators.

==> ACM Journal paper/chapters/1.Abstract.tex <==
\begin{abstract}
This paper presents a  multi-agent Deep Reinforcement Learning (DRL) framework for autonomous control and integration of renewable energy resources into smart power grid systems. In particular, the proposed framework jointly 
considers demand response (DR) and distributed energy management (DEM) for residential end-users.
DR has a widely recognized potential for improving power grid stability and reliability, while at the same time
reducing end-users' energy bills. However, the conventional DR techniques come with several shortcomings, 
such as the inability to handle operational uncertainties while incurring end-user disutility, 
which prevents widespread adoption in real-world applications. 
The proposed framework addresses these shortcomings by implementing DR and DEM based on real-time pricing strategy that is achieved using deep reinforcement learning.  
Furthermore, this framework enables the power grid service provider to leverage distributed energy resources (i.e., PV rooftop panels and battery storage) as dispatchable assets to support the smart grid during peak hours, thus achieving management  of distributed energy resources. Simulation results based on the Deep Q-Network (DQN) 
demonstrate significant improvements of the 24-hour accumulative profit for both prosumers and 
the power grid service provider, as well as major reductions in the utilization 
of the power grid reserve generators. 
\end{abstract}
% \vspace{-.5cm}


==> ACM Journal paper/chapters/2.Introduction.tex <==

\section{Introduction}
Advances in renewable energy generation and their availability as local 
energy resources in power systems facilitate a paradigm  shift  from  the traditional 
power consumers to the more resourceful energy \emph{prosumers}. 
A prosumer is an end-user with the ability to consume and produce energy ~\cite{5759167}. 
The number of prosumers is increasing as more households are proceeding to install 
Distributed Energy Resources (DERs), such as solar photovoltaic (PV) panels~\cite{ 7820171}.   
The premise of DERs is to provide economic and ancillary benefits 
to both prosumers and power grid service provider (SP). However, achieving the full potential of 
distributed household PV systems is challenging due to two main factors. 
\textbf{(1)} Currently, households with PV systems can only sell their excess energy during the 
daylight hours when the price of electricity is low.
\textbf{(2)} Current popular net-metering compensation schemes leave prosumers with limited 
economic benefits and little incentive to engage in grid support applications~\cite{corbett2018toward}.
As a result, existing models for integration of DERs into the grid create a non-profitable 
situation for both prosumers and SP~\cite{chakraborty2018analysis}. 
To mitigate these issues, integrating energy storage devices with DERs provides 
more flexibility for prosumers to participate in \emph{Demand Response} (DR)  programs~\cite{7063260}. Additionally, SP will accomplish higher profit through implementing distributed energy management (DEM) for residential DERs with bidirectional power flow. Therefore, a dynamic decision-making framework that combines DR and DEM can provide a win-win scenario for both prosumer and SP.

There are several works that utilize model-based control paradigms for microgrid and demand-side energy management problems, such as model predictive control (MPC)~\cite{gan2020data}, mixed-integer linear programming (MILP)~\cite{7114268}, dynamic and stochastic programming~\cite{farzaneh2019robust}, and alternating direction method of multiplier (ADMM)~\cite{7501891}. 
One key step for applying these techniques is to establish an accurate model that captures the dynamics of the microgrid and the interactions between various components with all the operational constraints. The model-based nature of these methods also exhibits limited generalization capabilities~\cite{dorokhova2021deep}.  Difficulties in handling nonlinear behavior, volatile renewable generations, and heterogeneity of the end-users represent other major shortcomings of these methods. In addition, it is more challenging for the SP to estimate the impact of its online pricing on customers' future behavior while considering the long-term performance of the microgrid. Overall, the conventional optimization techniques have to compute all the possible solutions on small-time horizons that results in high computational complexities and inefficiency for online use.

To overcome the aforementioned challenges, model-free Reinforcement Learning (RL) techniques are proven beneficial for demand-side energy management problems since they do not require an explicit model of the environment, which is challenging to acquire in practice. In this paper, we investigate the mutual interplay between participants and the different tasks in a residential microgrid. We propose a framework based on Deep Reinforcement Learning (DRL) for both SP and prosumers to enable dynamic decision-making.  A service provider agent (SPA) is deployed for solving the distributed energy management (DEM) problem in the microgrid by dynamically determining  the electricity buy price as a control parameter for optimization of the energy distribution. On the other side, the presence of prosumers provides a large-scale integration of DER schemes with different owners that tend to maximize their own profit without considering the other owners and the SPA performance. Here, the prosumer agent (PA) solves the prosumer energy management problem by determining the charge/discharge of the prosumer's battery installation. In summary, our main contributions are as follows:
% \vspace{-0.025in}
\begin{itemize}
 \item We develop a multi-agent DRL framework that interweaves the real-time energy management over the microgrid with the prosumer side real-time DR, using demand-dependent dynamic pricing for incentivizing prosumers' participation in DR.
  \item We show that the proposed DRL framework enables the service provider to leverage energy storages as dispatchable assets, while incentivizing the prosumers to actively participate in the program to support the grid activities.
 \item Our numerical results demonstrate that the proposed framework reduces the average daily bill for prosumers, while at the same time it provides higher profits for the grid service provider (SP) by leveraging distributed energy resources instead of tapping into traditional reserve generation facilities. 
\end{itemize}
The remainder of this paper is organized as follows. Section~\ref{sec:related_work} 
covers related work, followed by the system model and problem formulation in Section~\ref{sec:model}. 
Next, Section~\ref{sec:RLmodel} formulates the DRL framework, while Section ~\ref{sec:result} presents numerical results. Finally, Section \ref{sec:conclusion} concludes the paper. 

==> ACM Journal paper/chapters/3.Relatedwork.tex <==
\section{Related work}
\label{sec:related_work}

% \mycomment{YD: I think the related work section could use some organization and precision by grouping similar works together}
% \mycomment{Alex: It may be good to go back to using in-line subtitles to label the different kinds of related works. It may be easier to follow and you can remove quite a few connection words such as furthermore, moreover, etc.}
A multitude of prior works use RL in the context of power systems, mainly to locate optimal pricing. 
For instance, 
% a bidding strategy for an agent-based local microgrid was proposed in~\cite{7300459} 
% where each agent is responsible for trading electricity with other agents and maximizing their profit 
% in a local energy market with no grid connection. 
constrained energy trading between end-users was investigated in~\cite{wang2016reinforcement}.
% where adaptive RL was used to converge the bidding problem between participants. 
A hierarchical electricity 
market with bidding over wholesale and retail using RL was proposed 
in~\cite{xu2019deep}, while in~\cite{liang2020agent} a DDPG algorithm was used to solve the bidding problem 
of several generation companies. Moreover, RL have been widely employed for energy management optimization~\cite{foruzan2018reinforcement, 123456}. In~\cite{foruzan2018reinforcement}, the authors proposed a multi-agent distributed energy management framework with time-of-use pricing for a microgrid energy market with a centralized battery pack and renewable generation. 
% They used a Q-table algorithm with time-of-use pricing for solving the distribution optimization problem. 
In this work, we propose a dynamic pricing scheme with DQN for distributed battery and PV setup penetration. In~\cite{123456}, RL methods were utilized to manage the energy in a multi-microgrid system. 










% A multitude of prior works use RL in the context of power systems mainly to locate optimal pricing. 
% For instance, a bidding strategy for an agent-based local microgrid was proposed in~\cite{7300459} 
% where each agent is responsible for trading electricity with other agents and maximizing their profit 
% in a local energy market with no grid connection. 
% On the other hand, several works used RL by focusing on the single objective of 
% minimizing the cost of generation~\cite{8306311 ,9255238,dai2019distributed}. 
% In ~\cite{8306311}, Liu \emph{et al.} proposed a cooperative reinforcement learning approach 
% to solve the ED problem in microgrids with distributed generation resources and energy storage systems 
% with the goal of optimizing the cost of microgrid operations as well as satisfying the power constraints. 
% %which is not considered prosumers. 
% % In \cite{9255238},  the ED problem has been solved for a simple power system model. 
% Dai \emph{et al.}~\cite{dai2019distributed} also deployed reinforcement learning to solve the dynamic 
% economic dispatch problem to find the optimal output of each unit. 
% A multi-agent RL method with the objective of minimizing both fuel cost and emission in the 
% traditional power system model without renewable resources is proposed in~\cite{mannion2016dynamic}. 
% In \cite{8957677}, a deep reinforcement learning algorithm is proposed to obtain economic dispatch 
% in virtual power plants that are part of distributed energy resources, however, 
% the objective was still minimizing the operating cost of distributed generation (DG) resources 
% including photovoltaic and wind turbine. Although these prior efforts use RL in power systems 
% to locate optimal pricing, they do not include the newly arising entity covered in our work, 
% specifically the prosumers. 

Other research projects have addressed the interactions between retailer/SP and end-users. 
For example, \cite{samadi2014real} investigated a gradient-based method to minimize the 
aggregate load demand by assuming the presence of consumption scheduling devices on the users' side.   
Furthermore, works such as \cite{jia2016dynamic, yu2018incentive,8490840} leveraged the Stackelberg game
% . 
% Specifically, \cite{jia2016dynamic} used a Stackelberg game 
to model and maximize 
the retailer profit and minimize the payment bill of its customers. 
The authors included renewable energy generation on the retailer side, which is different from our model 
with distributed PV installations across prosumers. 

% \emph{Related Work on Demand Response:} 
% The conventional time-based DR approaches, such as the real-time pricing methods, mostly focus on altering the preferred electricity consumption pattern of the consumer, e.g. 
% by 
% % changing the temperature set point on air conditioning systems or 
% delaying the use of major appliances, in order to shift their load to off-peak hours.  However, these approaches lead to the dissatisfaction of consumers and therefore they have not been widely adopted thus far \cite{pinson2014benefits , haider2016review}. In contrast, our proposed prosumer side DR algorithm does not alter the consumption pattern of the households (no disutility).  Rather, it achieves cost savings by altering the households' power demand pattern, using the flexibility provided by energy storage coupled with PV generation.

% \cite{chen2013mpc} proposed a  model predictive control (MPC) based for appliance scheduling scheme of home energy management system to minimize consumer energy cost which does not consider the grid side. 


%Similarly, Stackelberg game was adopted in \cite{yu2018incentive} to model and analyze decision making components across the  service provider, and conventional and industrial consumers, i.e., no prosumer was considered.

%In \cite{zhang2017robust}, the overall economic benefits of operators and customers are optimized with price-based demand response. However, no energy storage and renewable energy are included in this model. 
% A two-stage robust optimization (TSRO) and column-and-constraint generation (C$\&$CG) algorithm is employed to ensure the optimization results are robust against all uncertainties however there is no energy storage and renewable energy in the model. 
On a different note, \cite{wang2020deep} developed a DRL-based load scheduling 
algorithm with a time-of-use scheme to reduce the peak load demand and the operation cost for the 
distribution system, however without considering prosumers. In~\cite{chung2020distributed} the interaction between households and the aggregator was modeled to jointly solve the energy scheduling consumption and preserving privacy for the households by using policy gradient RL method.
Furthermore, \cite{9281326} developed a home energy management system (HEMS) using Actor-Critic technique based on adaptive dynamic programming.
% that focuses on the consumer's dissatisfaction in a conventional setup and 
% without any renewable resources. 
Likewise, in \cite{7401112}, an energy management DR using RL adjusts 
the consumption plan for thermostatically controlled loads. 
%In \cite{7792709}, batch reinforcement learning technique is used for water heater consumption control using auto-encoder network to reduce the dimensionality of the state-space.
% The authors in \cite{8928284} investigated a DR problem for household heating system and electric water heater by applying a combination of two neural networks (convolutional and LSTM) and RL, and they did not consider renewable resources and energy storage for consumers.
Along the same lines, \cite{xu2020multi} proposed a framework for home energy management based 
on RL to minimize the electricity bill as well as DR-induced dissatisfaction costs for end-users. 
Their method considered proliferation of rooftop PV systems but did not consider
home energy storage systems. Moreover, \cite{bahrami2020deep} proposed a 
DRL approach to reduce peak load and household cost by load scheduling in an IEEE 33-bus test feeder with 
32 consumers. They demonstrated 33$\%$ reduction in peak load and 13$\%$ reduction in households' 
daily cost, without considering any storage system.
It is also worth noting that these works \cite{wang2020deep,7042790,7401112, 8928284,xu2020multi,bahrami2020deep} do not consider the grid side and only propose optimization algorithms for end-users.
% \mycomment{AB: How is our work different from these works?}

% Energy storage system has not been considered in none of the aforementioned researches which in our latest work \cite{Ghasemi} has shown that can be an effective parameter to improve the system efficiency in terms of reducing costs.
%Although some of the aforementioned works have considered the penetration of PV generations, none of them considered battery capabilities.
% \vspace{-0.1in}


% Both retailer and end-users profits maximization  has been studied in \cite{dehghanpour2016agent,lu2019incentive,DynamicPrice,11Dynamic}. 
The studies in \cite{dehghanpour2016agent} and \cite{lu2019incentive} proposed a hierarchical agent-based framework 
% for implementing a price-based DR program 
to maximize both retailer and customers profits. %The study reported in \cite{dehghanpour2016agent} used Q-learning for decision making problem in lower level side (end-user) and linear and ANN model model for upper level side (retailer) was used and their model can be used for load shaving as well.  
An RL-based DR is proposed in \cite{DynamicPrice} for the energy consumption scheduling problem that can work without prior information and leads to reduced system costs. Also, in \cite{11Dynamic} both service provider profit and consumers' cost are considered to find the optimal retail price. However, unlike our effort, the works presented in \cite{dehghanpour2016agent,lu2019incentive,DynamicPrice,11Dynamic} only consider regular electricity consumers, rather than prosumers with generation and storage capabilities. 
In contrast to these efforts, we model a microgrid that consists of both consumers and prosumers that are equipped with battery storage. As a result, the proposed multi-agent DRL framework achieves DR with dynamic pricing and distributed energy management for a microgrid with large-scale rooftop PV panels and energy storage system.
Table~\ref{tab:relatedwork} compares our work 
with the previous related work. 


\begin{table}
%  	\centering
 		\caption{Taxonomy of Related Work on Management of Distributed Energy Resources. (\Checkmark : Considered, ---: Not Considered ) }
 	\resizebox{\columnwidth}{!}{
  	\begin{tabular}{@{}lccccc@{}}\toprule
  	\textbf{Reference} & \textbf{Energy management } & \textbf{Retailer/end-user} & \textbf{Renewable penetration}
  	& \textbf{Energy storage} & \textbf{RL} \\
  	 & \textbf{DR} & \textbf{profit optimization}  & \textbf{consideration} & \textbf{consideration}  & \textbf{algorithm}\\
  	\midrule \cite{dehghanpour2016agent},\cite{DynamicPrice},\cite{11Dynamic} & \Checkmark & \Checkmark & --- & --- &\Checkmark \\
  	\cite{yu2018incentive},\cite{8490840},\cite{chung2020distributed},\cite{lu2019incentive}& \Checkmark & \Checkmark  & --- & --- & ---\\ 
  	\cite{xu2020multi} & ---& \Checkmark& \Checkmark  & --- & \Checkmark \\
  	\cite{wang2020deep}, \cite{bahrami2020deep} & --- & \Checkmark & --- & --- & --- \\
  	\cite{jia2016dynamic} & \Checkmark & --- & --- & \Checkmark & \Checkmark \\
  	Our proposed framework & \Checkmark &  \Checkmark & \Checkmark & \Checkmark  & \Checkmark \\ 
 	\bottomrule
 	\end{tabular}
 	}
 	\vspace{-0.1in}
 	\label{tab:relatedwork}
 \end{table}


==> ACM Journal paper/chapters/4.ProblemFormulation.tex <==
\section{Microgrid Model and Problem Formulation}\label{sec:model}

\begin{figure}[t]
\centering
\includegraphics[scale=0.5, trim=1.05cm 0.5cm 0.9cm 0.5cm, clip]{figures/caseStudy.pdf}
\caption{Proposed microgrid system architecture that consists of generation facilities, traditional consumers, and prosumers that are equipped with solar rooftop panels and energy storage and deep reinforcement learning agents. Grid and prosumers are equipped with deep reinforcement learning agents to dynamically adjust their policies in terms of buy/sell prices and power injection.}
\vspace{-0.12in}
\label{fig:system-model}
\end{figure} 
% \vspace{-0.6in}
% In this section, we define a microgrid consist of prosumers with access to PV resources and storage system followed by problem formulation for prosumers as well as power grid service provider. 
The envisioned microgrid model is shown in  Figure~\ref{fig:system-model}. 
On the end-user side, the microgrid consists of regular consumers as well as prosumers that are equipped with PV panels, battery, and an intelligent agent.
% -------------------------New Line---------------------
The presence of consumers ensure that the microgrid always has energy deficiency. The conventional generation units are connected to the microgrid to meet the deficiency. The base generation units have low cost for the service provider but if their capacity is not enough, the reserve and the more expensive generation facilities will be dispatched to meet the real-time microgrid demand~\cite{goodarzi2022evaluate}. Without loss of generality, this paper forgoes the ramp rate constraints of the generation facilities.
% -------------------------New Line---------------------
The agent decides on whether to consume the excess energy generated by the PV system, store it in the battery, or sell it to the grid. On the other side, the SP is responsible 
for dispatching power to the loads from various generation facilities, including distributed energy resources of prosumers. 


In this paper, distributed energy management and demand response optimization problems are defined for the SP and prosumers,  respectively. On the grid side, the SP is 
engaged in energy management with the objective of improving its own profit. On the household side, prosumers engage in DR 
with the goal of reducing their daily electricity bill. The complex interactions between the two sides 
denote the joint DEM-DR approach proposed in this paper. 
% This incurs some cost when buying the energy from prosumers. This cost depends on the \$/kWh price of buying electricity from prosumers, referred to as buy price  $\left(\rho_b\right)$  hereinafter. 
% Currently, grid operators buy the electricity from the prosumers at wholesale prices, but sell the electricity back to them at retail prices, referred to as sell price $\left(\rho_s\right)$ hereinafter, which are typically much higher than the wholesale prices.








%This response will determine the action applied to the battery storage in terms of charge or discharge. 
%Next, we formulate these two optimization problems.  

%we are envisioning prosumer setups that integrate battery energy storage and an intelligent energy management system.  The energy management system decides on whether to consume the excess energy generated by the PV system, store it in the batteries, or sell it to the grid. This enables prosumers to store their excess energy during the off-peak hours when the buy price is set lower by the grid, and sell it to the grid during the peak hours when the buy price is set higher. This will provide an opportunity for the prosumers to reduce their daily bills while participating in grid support applications.

%Next, we formulate the optimal power flow problem with the goal of reducing the prosumers' daily bill and also to minimize the cost of delivered power by identifying an optimal schedule for operating level of each generation units.

%we propose the following optimization problem for the jth prosumer

%\mh{something missing here?}
%\mh{Connection of this paragraph with the previous paragraph is not clear.}

%The goal of optimal power flow is to minimize cost of delivered power by identifying an optimal schedule for operating level of each generation units. 
%Which is formulated with $N_g$ generators, each with unit operating cost of $F_i{(P_{G_i})}$ as,
%\begin{equation}\label{eq:1}
%\mathbf{Minimize}{{\ \ \ F}_T = \ \sum_{i=1}^{N_g}{F_i\left(P_{Gi}\right)}}.
%\end{equation}
%While in smart grid the optimal operation will be ensured only when demand side constraint are standardize to maximize consumer welfare objective. So, price responsive demand can be a good solution to find the optimal operation. 
%The goal of traditional ED is to minimize the total cost of delivered power within confines of a balancing authority area (BAA) by identifying an optimal schedule for operating level of each generation unit that leads to a minimized total generation cost.  Moreover, the objectives of ED are typically further expanded to target minimization of a litany of other important functions such as transmission loss, deviation from target schedule, emissions, control shift in case of violations, etc.  In its simplest form the ED problem for a system with $N_g$ generators, each with unit operating cost of $F_i{(P_{G_i})}$, is formulated as a minimization problem for total generation cost of $F_T$ as,



%This optimization problem is subject to various operation and safety related constraints such as the grid power balance, power flow constrains, generator units’ ramp rate constraints, bus voltage magnitude constraints, minimum and maximum power output constraints for each generation unit, etc. Quadratic approximation or piecewise linear approximation are typically used for modeling the generation unit operating cost $F_i\left(P_{G_i}\right)$.  The power balance constraint is typically formulated as,     
%\begin{equation}\label{eq:2}
%P_D-P_{loss}-\sum_{i=1}^{N_g}\left(P_Gi\right)=0,
%\end{equation}
%where $P_D=\sum_{L=1}^{N_h+N_c}{P_{d_L}}$ is the total load demand which $N_h$ is number of prosumers and $N_c$ is number of consumers, and $P_{loss}$ is the total transmission loss over the network.  The simplified optimization problem in \ref{eq:1} and \ref{eq:2}, can be described using the following Lagrange function, 
%\begin{equation}\label{eq:3}
%L=\sum_{i=1}^{N_g}{F_i\left(P_{Gi}\right)+\lambda.(P_D+P_{loss}-\sum_{i=1}^{N_g}P_{Gi})},
%\end{equation}
%where $\lambda$ is the Lagrangian multiplier.  The optimally condition then can be formulated as,
%\begin{equation}\label{eq:4}
%\frac{\partial F_i(P_i)}{\partial P_i}.\frac{1}{\left(1-\frac{\partial P_{loss}}{\partial P_i}\right)}=\lambda\ ,\ \ for\ i=1,2,\ldots,NG. 
%\end{equation}

%Although \ref{eq:4} is the result of simplifying the ED problem significantly by only considering power balance constraint, it is still very challenging to solve this nonlinear equation using conventional techniques because they might fail to find the global optimum, and also with increasing numbers of constraints and variable they perform poorly in terms of speed. \mh{Connection of this part with the previous discussion is not clear. The problem formulation does not seem to be complete at this point that we are talking about Lagrange multiplier technique.\response{??}}




%\subsection{Economic Dispatch in a Microgrid with Prosumers }

%This leaves prosumers with very limited economic benefits and little incentive to engage in grid support applications. Therefore, in this work, we envision an electricity market in which, the buy price is dynamic variable set by the grid in real time and used for incentivizing the prosumers to participate in power balancing and providing various other grid support services. 

%In this power market, although buying electricity from prosumers incurs additional cost for the grid, nonetheless, it can reduce the operating cost of generation units, because some portion of the power required to maintain the power balance is delivered by the prosumers, bringing down the required power output level of generators.




%Thus, power flow will be managed in order to improve the power grid's profit and reduce the prosumer's daily bill.

%So, these two factors will be added subject to power balance equation 


%\AS{Again this is confusing because there are several power balance equations. In my opinion if the optimization problems define at first then adding two different parts make sense }.




% \subsubsection{\textbf{Service provider economic dispatch}}
% The goal of traditional ED problem is to meet the load demand while minimizing the SP cost expressed as, 
% \vspace{-0.08in}
% \begin{equation}\label{eq:ED}
% {\rm min}\ {\rm F}_{Total}=\sum_{i=1}^{N_g}{{\rm F}_{G_i}(T)},
% \vspace{-0.07in}
% \end{equation}
%  where ${\rm F}_{Total}$ is the total cost of power generation over a time horizon  $T$, and ${\rm F}_{G_i}$ is the cost of $i^{th}$ generation facility~\cite{ongsakul2013artificial}. Given that $P_{D}(t)$ is the total load demand and $P_{G_i}(t)$ is $i^{th}$ generator power at time $t$, the cost optimization is carried out subject to transmission and operational constraints, the most fundamental of which is the grid power balance, 
% \vspace{-0.07in}
% \begin{equation}
%     \sum_{i=1}^{N_g}{P_{G_i}}(t) - P_D(t) = 0.
% \end{equation}

%\begin{equation}\label{eq:conventionalED}
%\left\{ {\begin{array}{*{20}{c}}
%{{\rm{minimize}}\,\,\,\,\,\,\,\,\,{{\mathop{\rm %F}\nolimits} _{{G_1}}}(T) + {{\mathop{\rm %F}\nolimits} _{{G_2}}}(T) + ... + {{\mathop{\rm %F}\nolimits} _{{G_{{N_g}}}}}(T)}\\
%{{\rm{subject}}\,{\rm{to}}:\,\,\,\,\,\,\,\,\,\,\,%\,\,\,\,\,{P_{{G_1}}} + {P_{{G_1}}} + ... + %{P_{{G_1}}} = {P_{D}}}
%\end{array}} \right. 
%\vspace{0.05in}
%\end{equation}
% Emergence of prosumers alters some of the fundamental assumptions for conventional optimal power flow (OPF) formulations. 
% \vspace{0.01in}
\textbf{Service Provider Energy Distribution Model:} In the presence of prosumers, the DEM problem of the microgrid evolves into a much more complex problem since the prosumers also appear as generation facilities in certain time periods due to injection of power into the grid. Hence, in this paper, the DEM formulation is defined as follows \vspace{-0.1in},
% \subsubsection{\textbf{Power Grid Profit Improvement}}
% From the power grid point of view, the cost trade-off problem will result in a much more complex problem, because in addition to the generation facilities, prosumers will also inject power to the power grid. We consider the following formulation for the grid profit in presence of prosumers,
%As a result, the conventional generation minimization formulation in \ref{eq:1} for ED, will be transformed to a much more complicated cost trade-off problem. As such, in this work, we propose the following formulation for the ED problem in presence of prosumers,
% \begin{equation}\label{eq:Grid Profit}
% {\ \ \ \psi}^G_T=\ R_G\left(P_D\right)-\left\{\sum_{i=1}^{N_g}{F_i\left(P_{G_i}\right)}+\sum_{j=1}^{N_h}{F_j\left(P_{H_j}\right)}\right\},
% \end{equation}
% \vspace{-0.2in}
% \begin{equation}\label{eq:Grid Profit}
% {{{\Psi}}_G}(T) = {{\mathop{\rm R}\nolimits} _G}(T) - \left\{ {\sum\limits_{i = 1}^{{N_g}} {{{\mathop{\rm F}\nolimits} _{{G_i}}}(T)}  + \sum\limits_{j = 1}^{{N_p}} {{{\mathop{\rm F}\nolimits} _{{H_j}}}(T)} } \ri ght\},
% \vspace{-0.05in}
\begin{align}
   &\max_{\rho_b}
   \begin{aligned}[t]
      & \ \ {{{\Psi}}_G}(T)={{\mathop{\rm R}\nolimits} _G}(T) - \left\{ {\sum\limits_{i = 1}^{{N_g}} {{{\mathop{\rm F}\nolimits} _{{G_i}}}(T)}  + \sum\limits_{j = 1}^{{N_p}} {{{\mathop{\rm F}\nolimits} _{{H_j}}}(T)} } \right\} \label{eq:Grid Profit}
   \end{aligned} \\
   &\text{Subject to:} \notag \\
   & \sum\limits_{i=1}^{{N_g}} {{{\mathop{\rm F}\nolimits} _{{G_i}}}(T)}  = \sum\limits_{i=1}^{{N_i}} {{{\mathop{\rm F}\nolimits} _{{B_i}}}(T)}  + \sum\limits_{i=1}^{{N_r}} {{{\mathop{\rm F}\nolimits} _{{R_i}}}(T)} \label{eq:Reserve}, \\
   & {{\mathop{\rm R}\nolimits} _G}(T) = \int\limits_0^T {{P_D}(t).{\rho _s}(t)dt} \label{eq:Grid revenue}, \\
   & {{\mathop{\rm F}\nolimits} _{{H_j}}}(T) = \int\limits_0^T {{P_{{H_j}}}(t)} .{\rho _b}(t)dt\,\,\,\,\,\,\,\,\rm{for}\,\,\,{P_{{H_j}}}(t) \ge 0 \label{eq:Prosumer injection}, \\
   & {P_D}(t)  = \sum\limits_{i = 1}^{{N_g}} {{(P_{{G_i}}}(t)- P_{{loss}_i}(t))}  + \sum\limits_{j = 1}^{{N_p}} {{P_{{H_j}}}(t)} \label{eq:Power balance grid}, \\
   & P_{{loss}_i}= \beta_i \times P_{G_i}^2(t), \\
   & P_{{G_i}}^{\min } \le {P_{{G_i}}}(t) \le P_{{G_i}}^{\max }\,\,\,\,{\rm{for}}\,\,i = 1,2,...,{N_g} \label{eq:utility_limit},
 \end{align}
% \begin{align}
% \max_{\rho_b}
% & & {{{\Psi}}_G}(T)={{\mathop{\rm R}\nolimits} _G}(T) - \left\{ {\sum\limits_{i = 1}^{{N_g}} {{{\mathop{\rm F}\nolimits} _{{G_i}}}(T)}  + \sum\limits_{j = 1}^{{N_p}} {{{\mathop{\rm F}\nolimits} _{{H_j}}}(T)} } \right\}, \label{eq:Grid Profit} \\
% \text{subject to:}
% & & \sum\limits_{i=1}^{{N_g}} {{{\mathop{\rm F}\nolimits} _{{G_i}}}(T)}  = \sum\limits_{i=1}^{{N_i}} {{{\mathop{\rm F}\nolimits} _{{B_i}}}(T)}  + \sum\limits_{i=1}^{{N_r}} {{{\mathop{\rm F}\nolimits} _{{R_i}}}(T)} \label{eq:Reserve}, \\
% & & {{\mathop{\rm R}\nolimits} _G}(T) = \int\limits_0^T {{P_D}(t).{\rho _s}(t)dt} \label{eq:Grid revenue}, \\
% & & {{\mathop{\rm F}\nolimits} _{{H_j}}}(T) = \int\limits_0^T {{P_{{H_j}}}(t)} .{\rho _b}(t)dt\,\,\,\,\,\,\,\,\rm{for}\,\,\,{P_{{H_j}}}(t) \ge 0 \label{eq:Prosumer injection}, \\
% & & {P_D}(t)  = \sum\limits_{i = 1}^{{N_g}} {{(P_{{G_i}}}(t)- P_{{loss}_i}(t))}  + \sum\limits_{j = 1}^{{N_p}} {{P_{{H_j}}}(t)} \label{eq:Power balance grid}, \\
% & & P_{{loss}_i}= \beta_i \times P_{G_i}^2(t), \\
% & & P_{{G_i}}^{\min } \le {P_{{G_i}}}(t) \le P_{{G_i}}^{\max }\,\,\,\,{\rm{for}}\,\,i = 1,2,...,{N_g} \label{eq:utility_limit},
% \end{align}
where ${{{\Psi}}_G}(T)$ denotes the SP profit over a time horizon of $T$, and ${{{\rm R}}_G}(T)$
is SP revenue as a result of selling electricity to the loads, which is calculated by Equation \eqref{eq:Grid revenue} where ${P_D}(t)$ and ${\rho_s}(t)$ denote the total system demand and electricity sell price at any given time, respectively. ${\rm F}_{G_i}(T)$ is the cost of generation unit $i$ defined as the quadratic function of $P_{{G_i}}$, which means ${\rm F}_{G_i}(P_{{G_i}})={a_i}P_{{G_i}}^2+{b_i}P_{{G_i}}+{c_i}$ where $a_i$, $b_i$, and $c_i$ are fitting parameters and $P_{{G_i}}$ is the amount of power purchased from generation unit $i$ \cite{ongsakul2019artificial}. This cost consists of the cost of base generation units ${{{\mathop{\rm F}\nolimits} _{{B_i}}}(T)}$ and cost of reserve generation units ${{{\mathop{\rm F}\nolimits} _{{R_i}}}(T)}$ in Equation \eqref{eq:Reserve} where $N_i$ and $N_r$ are the number of base and reserve generation facilities, respectively. $N_g$ is the number of all generation facilities. If the power demand exceeds the amount of base generation, the overall cost will be significantly higher because procuring reserve power is more costly. ${\rm F}_{H_j}{(T)}$ is the cost of buying electricity from the $j^{th}$ prosumer and calculated by Equation \eqref{eq:Prosumer injection} where ${P_{{H_j}}}(t)$ and ${\rho_b}(t) $ denote the power injected by the $j^{th}$ prosumer and electricity buy price, respectively. Equation \eqref{eq:Power balance grid} illustrates the total generation and total demand power balance requirement, which needs to be maintained at any given time slot $t$. $N_p$ and $N_c$ denote the number of prosumers and consumers, respectively. $P_{{loss}_i}$ denotes the losses induced by generation unit $i$, where $\beta_i$ is the loss coefficient \cite{7387777}. In addition, the power output of each generation unit must not exceed its operation limits, which are described in Equation \eqref{eq:utility_limit}.

The SP's goal is to maximize its profit. To do so, the SP dynamically changes the buy price to incentivize the prosumers to sell their excess energy to the grid, especially during the peak demand hours. Hence, the control variable in DEM problem is the buy price  $\rho_b(t)$. 


\textbf{Prosumer Side Demand Response Model:}
The objective of the prosumers is to minimize their daily electricity bill by engaging in DR as a response to the dynamic buy price controlled by the SP. Therefore, the prosumer side profit maximization is formulated as follows\vspace{-0.1in},
%In order to provide beneficial situation for prosumers as well, maximizing prosumers local profit is an objective in our problem. In this work, we consider the following optimization problem for the $j^{th}$ prosumer




\begin{align}
  &\max_{P_{b_j}}
  \begin{aligned}[t]
      & \ \ {{{\Psi }}_{{H_j}}}(T)={{\mathop{\rm F}\nolimits} _{{H_j}}}(T) + \boldsymbol{\mathbbm{1}}_{\{P_{H_j}(t) < 0\}} \times {{\mathop{\rm C}\nolimits} _{{H_j}}}(T) \label{eq:Prosumer profit}
  \end{aligned} \\
  &\text{Subject to:} \notag \\
  & {{\mathop{\rm C}\nolimits} _{{H_j}}}(T) = \int\limits_0^T {{P_{{H_j}}}(t)} .{\rho _s}(t)dt\,\,\,\,\,\,\,\,\rm{for}\,\,\,{P_{{H_j}}}(t) < 0 \label{eq:prosumer_cost},\\
  & {{\mathop{\rm F}\nolimits} _{{H_j}}}(T) = \int\limits_0^T {{P_{{H_j}}}(t)} .{\rho _b}(t)dt\,\,\,\,\,\,\,\,\,\,\rm{for}\,\,\,{P_{{H_j}}}(t) \ge 0, \nonumber \\
  & {P_{{H_j}}}(t) = {P_{P{V_j}}}(t) - {P_{b_j}}(t) - {P_{{C_j}}}(t) \label{eq:Power balance prosumer}, \\
  & SoC_{{b_j}}^{\min } \le \frac{1}{{{C_{{b_j}}}}}\int\limits_0^t {{P_{b_j}}(\tau )d\tau } + So{C_{{b_j}}}(0) \le SoC_{{b_j}}^{\max } \label{eq:batttery_limit}, \\
  & P_{b_j}^\text{max, dis} \le P_{b_j}(t)\le P_{b_j}^\text{max, charge} \label{eq:battery charge/discharge constraint}, \\
  & 0\le\ P_{PV_j}\left(t\right)\le\ P_{{PV}_j}^\text{max} \label{eq:PV constraint}, \\
  & \left|{P}_{H_j}(t)\right|\le\ P_{H_j}^\text{max} \label{eq:injection constraint}, \\
  & So{C_{{b_j}}}(0),\quad SoC_{{b_j}}^{\min },\quad P_{H_j}^\text{max}\geq0, \notag
\end{align}
% {\small
% \begin{align}
% & \max_{P_{b_j}}
% & & {{{\Psi }}_{{H_j}}}(T)={{\mathop{\rm F}\nolimits} _{{H_j}}}(T) + \boldsymbol{\mathbb{1}}_{\{P_{H_j}(t) < 0\}} \times {{\mathop{\rm C}\nolimits} _{{H_j}}}(T) \label{eq:Prosumer profit} \\
% & \text{subject to:}
% & &{{\mathop{\rm C}\nolimits} _{{H_j}}}(T) = \int\limits_0^T {{P_{{H_j}}}(t)} .{\rho _s}(t)dt\,\,\,\,\,\,\,\,\rm{for}\,\,\,{P_{{H_j}}}(t) < 0 \label{eq:prosumer_cost}, \\
% & & & {{\mathop{\rm F}\nolimits} _{{H_j}}}(T) = \int\limits_0^T {{P_{{H_j}}}(t)} .{\rho _b}(t)dt\,\,\,\,\,\,\,\,\,\,\rm{for}\,\,\,{P_{{H_j}}}(t) \ge 0 \label{eq:Prosumer injection}, \nonumber \\
% & & & {P_{{H_j}}}(t) = {P_{P{V_j}}}(t) - {P_{b_j}}(t) - {P_{{C_j}}}(t) \label{eq:Power balance prosumer}, \\
% & & & SoC_{{b_j}}^{\min } \le \frac{1}{{{C_{{b_j}}}}}\int\limits_0^t {{P_{b_j}}(\tau )d\tau } + So{C_{{b_j}}}(0) \le SoC_{{b_j}}^{\max } \label{eq:batttery_limit}, \\
% & & & P_{b_j}^\text{max, dis} \le P_{b_j}(t)\le P_{b_j}^\text{max, charge} \label{eq:battery charge/discharge constraint}, \\
% & & & 0\le\ P_{PV_j}\left(t\right)\le\ P_{{PV}_j}^\text{max} \label{eq:PV constraint}, \\
% & & & \left|{P}_{H_j}(t)\right|\le\ P_{H_j}^\text{max} \label{eq:injection constraint},\\
% & & & So{C_{{b_j}}}(0),\quad SoC_{{b_j}}^{\min },\quad P_{H_j}^\text{max}\geq0, \notag
% \end{align}\vspace{-0.2in}}
where ${\Psi}_{H_j}{(T)}$ is the profit of the $j^{th}$ prosumer and  $C_{H_j}{(T)}$ is the cost of buying electricity from the grid over the time horizon $T$, which is described by Equation \eqref{eq:prosumer_cost}. ${{\mathop{\rm F}\nolimits} _{{H_j}}}(T)$ describes the prosumer $j$ revenue as a result of selling power to the grid and is calculated by Equation \eqref{eq:Prosumer injection}. Each prosumer has an internal household-scale power system with a power balance equation of its own that needs to be satisfied at all times. This is formulated by Equation \eqref{eq:Power balance prosumer} where $P_{PV_j}$, $P_{b_j}$ and $P_{C_j}$ are the amount of PV generation, battery charging/discharging power, and power consumption of the $j^{th}$ prosumer, respectively. According to Equation \eqref{eq:Power balance prosumer}, $P_{H_j}$ can take a positive or negative value depending on the amount of PV generation and battery charge or discharge action. A positive (negative) value means the prosumer $j$ injects (purchases) power to (from) the grid. Hence, $\boldsymbol{\mathbbm{1}}_{\{P_{H_j}(t)<0\}}$ is one/zero when the injected power from prosumer $j$ is negative/positive. The state of charge of each prosumer battery should be maintained within a safe operational range as illustrated in Equation \eqref{eq:batttery_limit} where $C_{b_j}$ is the nominal battery capacity and ${SoC}_{b_j}\left(0\right)$ represents the initial state of charge of the battery. ${SoC}_{b_j}^{\min}$ and ${SoC}_{b_j}^{\max}$ are the lowest and highest allowable state of charge for the battery, respectively. Furthermore, the charging and discharging power of the battery is limited as Equation \eqref{eq:battery charge/discharge constraint}, where $P_{b_j}^\text{max, charge}$ and $P_{b_j}^\text{max, dis}$ are the maximum charge/discharge power ratings of the battery. The constraint in Equation \eqref{eq:PV constraint} is imposed by the physical limitations of the size of the PV system and shows that the amount of PV generation is limited by the $P_{{PV}_j}^\text{max}$. Dynamic power injection into the grid might cause instability in some cases. Thus, the maximum allowable power injection is limited by Equation \eqref{eq:injection constraint}.

\begin{figure}[t]
\centering
\includegraphics[scale=0.42, trim=5.5cm 5cm 5.1cm 5cm, clip]{figures/Fig_RL3.png}
% \vspace{-.2in}
\caption{Implemented Reinforcement Learning framework}
\label{fig:RL}
\end{figure}

% It should be noted that there is no interaction between the prosumers such that their goals are to maximize their local profit regardless of other prosumers' performance. We have allocated a local agent to each prosumer to account for local observations.
In this paper, the formulated DR method is different from the conventional time-based DR, such as Real-Time Pricing (RTP) methods \cite{samadi2014real}.
Conventionally, RTP approaches rely on dynamically changing the electricity sell price to motivate the customers to alter their energy use profile, while the proposed DEM-DR algorithm relies on dynamically changing the buy price instead of the sell price. This potentially incentivizes prosumers to participate in the program without any customer dissatisfaction. At any given time slot $t$, both aforementioned optimization problems must be solved at the same time. Dynamic SP pricing scheme in DEM-DR problem reinforces the need to implement the optimization problems in short intervals (e.g., 15 minutes).
% , which is time-consuming and computationally expensive. Also, renewable equipment and customers' behavior add more uncertainties to the problem, which is hard to implement in traditional optimization algorithms. Hence, to address the aforementioned issues we leverage model-free RL algorithm, to develop an online solution.
% Next, we present a reinforcement learning framework to solve the formulated DEM and DR problems. 
%Next, we present a reinforcement learning framework for making dynamic decisions at each time interval.
% After formulating the problem in the micro grid system, we want to implement this problem as a Markov Decision Process (MDP) and utilizing the agent-based reinforcement learning to solve our ED-DR problem.

==> ACM Journal paper/chapters/5.RL.tex <==
\section{Reinforcement Learning for DEM and DR}\label{sec:RLmodel}
Reinforcement Learning (RL) is a model-free machine learning technique that trains an agent to take optimal actions through repeated interactions with an environment.
% This interaction can be  modeled as a Markov Decision Process (MDP).  
The general RL framework consists of a set of states $\mathcal{S}$, a set of actions $\mathcal{A}$, a reward function $R$, and probability of transition between the states. The policy $\pi$ is a mapping from the states of the environment ($s^t$) to the actions ($a^t$), i.e., $\pi:\mathcal{S}\rightarrow\mathcal{A} $. 
% The value of policy $\pi$, denoted by $V^\pi(s^t)$, is the
% % expected cumulative 
% reward that the agent receives under policy $\pi$.
The agent's ultimate goal is to learn which action $a^t \in \mathcal{A}$ to take at each time instance $t$ to maximize its
cumulative reward over time.  The action $a^t$ results in reward $r^t$, and the environment transitions from the state $s^t$ to $s^{t+1}\in \mathcal{S}$.
%The set of repeated actions is collectively referred to as the policy $\pi^*$.

In this section, we use $t$ as superscript to denote discrete time slots. It should be noted that there is no interaction between the prosumers, such that their goals are to maximize their local profit regardless of other prosumers' performance.

% We have allocated a local agent to each prosumer to account for local observations. Although there is no direct power or information exchange between any two prosumers, the interaction between the SPA and PAs can be considered as a competitive game where the revenue of the prosumers in \eqref{eq:Prosumer profit} is a cost term for the SPA in  \eqref{eq:Grid Profit}. 
% such that when the agent follows that policy for all states, it gets the maximum expected cumulative reward.
% , i.e.,
% \begin{equation}\label{eq:Policy value}
% V^*(s^t) = \max_\pi V^\pi(s^t),
% \end{equation}

% \vspace{-.2in}
% \begin{figure}[H]
% \centering
% \includegraphics[scale=0.4, trim=0.5cm 0.5cm 0.5cm 0.5cm, clip]{figs/RL.pdf}
% \vspace{-.2in}
% \caption{A general reinforcement learning framework where an agent interacts with the environment. 
% % As a result of agent's action, the environment transitions to a new state, and. 
% The agent receives a reward commensurate with the merit of the action.}
% \label{fig:RL}
% \end{figure}
\vspace{-0.1in}
\subsection{Decision-Making Problem Formulation} 
% DRL Framework for the Proposed DEM-DR Problem
In order to tackle the optimization problems in Section \ref{sec:model}, we leverage a multi-agent DRL approach such that we define agent for the grid side SP and agents for the prosumer side with PV and battery storage capabilities. The $\text{SPA}$ is representative of the service provider agent, while $\text{PA}_j$ denotes the $j^{th}$ prosumer agent. Each agent observes the environment and subsequently takes an action, receiving a reward commensurate with the merit of the action. The agents will receive a reward through their action selection, which is profit maximization for SPA and electricity bill reduction for PA. Figure \ref{fig:RL} graphically demonstrates the interaction between the SPA and PA agent with the environment, their observation, and the action for each agent. 
\subsubsection{Service Provider Agent} 
The $\text{SPA}$ observes the cost of buying electricity (base and reserve generation) from $N_g$ generation facilities at time slot $t$, which is  denoted by ${\bf{F}}_G^t = [{\mathop{\rm F}\nolimits} _{{G_1}}^t,{\mathop{\rm F}\nolimits} _{{G_1}}^t,...,{\mathop{\rm F}\nolimits} _{{G_{{N_g}}}}^t]$. In addition, the $\text{SPA}$ observes the cost of buying electricity from $N_p$ prosumers denoted by ${\bf{F}}_H^t = [{\mathop{\rm F}\nolimits} _{{H_1}}^t,{\mathop{\rm F}\nolimits} _{{H_1}}^t,...,{\mathop{\rm F}\nolimits} _{{H_{{N_p}}}}^t]$, and the total power demand of the loads $P_D^{t}$ at the time slot $t$. Hence, environment states $s_{SPA}^t = \{ {\bf{F}}_G^t ,{\bf{F}}_H^t ,P_D^{t} \} \in \mathcal{S}_{SPA}$ are observable by the SPA. Subsequently, the SPA takes an action by adjusting the electricity buy price denoted by $a_{SPA}^t=\rho_b^t \in \mathcal{A}_{SPA}$, where $\mathcal{A}_{SPA}$ is the finite set of available actions for SPA, i.e., all the possible buy prices. 

The $\text{SPA}$ reward function is defined based on the grid profit, 
\vspace{-0.05in}
\begin{equation}\label{eq:SPA_reward}
r_{SPA}^t = P_D^t \times \rho _s^t - \sum\limits_{i = 1}^{{N_g}} {{\mathop{\rm F}\nolimits} _{{G_i}}^t - \sum\limits_{j = 1}^{{N_p}} {\boldsymbol{\mathbbm{1}}_{\{P_{H_j}(t)\geq0\}} \times P_{{H_j}}^t \times \rho _b^t}},
\end{equation}
where $r_{PSA}^t$ is the SPA reward at time slot t.
The value of ${\mathop{\rm F}\nolimits} _{{G_i}}^t$ is obtained using the incremental cost curve of the $i^{th}$ generation facility. Given the definition of the immediate reward, the ultimate goal for the SPA is to maximize the cumulative reward $R_{SPA}^t=\sum_{k=0}^{\infty}{\gamma^k r_\text{SPA}^{t+k+1}}$ over an infinite time horizon known as expected return,
% \vspace{-0.1in}
% \begin{equation}\label{eq:24}
%  R_{SPA}^t=\sum_{k=0}^{\infty}{\gamma^k r_\text{SPA}^{t+k+1}}\ ,
% \end{equation}
where $0\le{\gamma}\le1$ is the discount factor.


\subsubsection{Prosumer Agent}  
${PA}_j$ observes its own local parameters at each time slot $t$ including power consumption $P_{C_j}^t$, state of charge of the battery $SoC_j^t$, and the PV generation $P_{PV_j}^t$, as well as the electricity buy price $\rho_b^t$ which is the result of SPA action. Hence $s_{PA_j}^t = \{ P_{C_j}^t,SoC_j^t ,P_{PV_j}^t , \rho_b^t \} \in \mathcal{S}_{{PA}_j}$.
Subsequently, the charge/discharge command to the energy storage in prosumer $j$ is the action determined by $PA_j$, which is shown by $a_{PA_j}^t=P_{b_j}^t\in\mathcal{A}_{PA_j}$. 
In this case, $\mathcal{A}_{PA_j}$ is the finite set of available actions to $PA_j$.
The reward function for the prosumer agents is defined as,
\begin{equation}\label{eq:PA reward}
r_{P{A_j}}^t = \boldsymbol{\mathbbm{1}}_{\{P_{H_j}(t)\geq0\}}  \times P_{{H_j}}^t \times \rho _b^t + \boldsymbol{\mathbbm{1}}_{\{P_{H_j}(t) < 0\}} \times P_{{H_j}}^t \times \rho _s^t.
% \vspace{-0.2in}
\end{equation}

Similar to the SPA, the $PA_j$ tries to maximize its infinite-horizon accumulative reward $R_{{PA_j}}^t=\sum_{k=0}^{\infty}{{\tilde{\gamma}}_j^k r_{{PA_j}}^{t+k+1}}$,
% \begin{equation}\label{eq:25}
% R_{{PA_j}}^t=\sum_{k=0}^{\infty}{{\tilde{\gamma}}_j^k r_{{PA_j}}^{t+k+1}}\ ,
% \end{equation}
where $0\le\tilde{\gamma}_j\le1$ is the discount rate for $PA_j$.

\begin{figure}[t]
\centering
 \includegraphics[scale=0.34, trim=4.5cm 1cm 5cm 0.04cm, clip]{figures/Timeline5.png}
 \vspace{-0.3in}
 \caption{Timeline of interaction between the SPA and PA. At each time slot $t$, the SPA dynamically determines the buy price in Step 2 (based on collected information in Step 1), and the PA decides on injected power and changing the battery state of charge in Step 3. }
 \vspace{-0.1in}
 \label{Timelinel}
\end{figure}
% \vspace{-.2in}

% \begin{algorithm}[t]
%     \caption{Q-learning Algorithm}
% % 	\begin{varwidth}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
% 		\begin{algorithmic}[1]
% 			\State Initialize  $Q(s,a)$ to zero
% 			\For {each Episode} 
% 			\For {each Iteration} 
% 			\State $t: = t + 1$
% 			\State Choose action $a$ using policy derived from $Q$
% 			\State Act upon $a$, Observe reward $r$ and new state $s^{t+1}$
% 			\State Update $Q(s,a)$ using \eqref{eq:Q value}  \State $s^t:=s^{t+1}$
% 			\EndFor
% 			\EndFor
% 		\end{algorithmic}
% 		\label{alg1}
% % 	\end{varwidth}
% \end{algorithm}


The timeline of interactions between the SPA and PA agents is illustrated in Figure~\ref{Timelinel}. At a given time slot $t$, the SPA makes a decision first by determining the market electricity buy price ($a_{SPA}^t$) based on the complete information of the prices of electricity generation facilities and the electricity demand from the prosumers' agents. The SPA then receives a reward ($r_{SPA}^t$) for taking the action. Next, the PAs observe the sell and buy price, and make the decision ($a_{PA_j}^t$) in terms of changing the battery state of charge and receive a reward ($r_{P{A_j}}^t$) for that decision. Finally, the PAs inform the SPA about the demand and the injected power.  

% These steps include the SPA decisions on determining the electricity buy price, and the PA actions on charge/discharge of the battery. 


\vspace{-.1cm}
\subsection{Deep Q-Network Learning}
A systematic review of Deep Learning (DL) methods applied to the smart grid is provided in \cite{massaoudi2021deep}. Deep Reinforcement Learning is the combination of Deep Neural Networks (DNNs) and RL. In general, RL solutions can be divided into value- and policy-based algorithms. 
The value-based solutions are straight-forward to implement. 
% and tend to be understandable. 
The main value-based method is Q-learning. Due to the high dimensionality nature of the problem Deep Q-Network (DQN) agents, which can handle a large state space, are used to solve their respective Markov Decision Processes (MDPs) and maximize their accumulative rewards. In addition, since the action spaces of SPA and PAs are discrete, the DQN can be used for solving this problem. The transition formula of Q-learning is,
% \vspace{-0.2in}
\begin{align}\label{eq:Q value}
Q(s^t,a^t) \leftarrow  Q(s^t,a^t) + {\alpha}[r^{t + 1} + {\gamma}&\mathop{\max }\limits_{{a ^{t + 1}}} Q(s^{t + 1},a^{t + 1}) - Q(s^t,a^t)]\ ,
\end{align}
where $\alpha$ is the learning rate. Additionally, $\gamma$ is the discount factor, with a range of 0 to 1. If $\gamma$ is closer to zero, the agent prioritizes the immediate reward over long-term rewards. On the other hand, if $\gamma$ is closer to one, the agent places greater weights over the future rewards compared with the immediate reward. The estimated Q-values are used to find the optimal policy that maximizes the accumulative rewards. 
% that changes based on the trade-off between exploration vs exploitation to find the optimal policy.
%\mh{$\epsilon$ is used to trade-off exploration and exploitation}.
An $\epsilon$-greedy strategy is used to balance between exploration and exploitation, i.e., 
\begin{equation*}\label{eq:E greedy}
    {a^t}=\begin{cases}
        \arg \mathop {\max }\limits_{{a^t}} \,E\left[ {Q\left( {{s^t},{a^t}} \right)} \right] & \text{with probability} \ 1 - \epsilon, \\
    \text{random action} & \text{with probability} \  \epsilon, 
            \end{cases}
\end{equation*}
% \begin{equation}\label{eq:E greedy}
% {a^t}  = \left\{ \begin{array}{l}\arg \mathop {\max }\limits_{{a^t}} \,E\left[ {Q\left( {{s^t},{a^t}} \right)} \right]\,\,\,\,\,\,\,\,\,{\rm{with}}\,\,{\rm{probability}}\,\,1 - \varepsilon, \\{\rm{random}}\,\,{\rm{action}}\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,{\rm{with}}\,\,{\rm{probability}}\,\,\,\,\varepsilon. \end{array} \right.\
% \end{equation}
where the probability of random action is $\epsilon$ that decays from 1 to 0.01 over the training episodes in our simulations. 
% Algorithm 1 summarizes the Q-learning method. 
%\subsection{Collected Data}


==> ACM Journal paper/chapters/6.Numerical.tex <==
\section{Numerical Results}\label{sec:result}
% \subsection{Simulation Setup}
% \mycomment{Alex: Keep an eye on the spacing between the columns}
In this study, we leverage the grid and prosumers' agents to implement the proposed DEM-DR scheme referred to as \emph{Agent-Based} scheme. To demonstrate the efficacy of the proposed approach, we compare it with the \emph{Conventional} approach, which simply injects the excess power to the grid when the battery is fully charged.  The simulation parameters for DQN agents are tabulated in Table~\ref{tab:SimulationParam}. As previously mentioned, the set of buy prices is defined as $\mathcal{A}_{SPA}$, representing the action space of the service provider agent. We designate the action space for prosumers as follows, 
\begin{align}\label{eq:PAaction}
P_{{b_j}}^t = \begin{cases}
                P_{b_j}^{\text{max,charge} } &\text{Charge\ action,} \\
                0 &\text{No\ charge\ or\ discharge\ action,}\\
                 P_{{b_j}}^{\text{max,dis} }&\text{Discharge\ action.}
            \end{cases}
\end{align}
% \begin{equation}\label{eq:PAaction}
% P_{{b_j}}^t = \left\{ \begin{array}{l}P_{b_j}^{\max,charge }\,\,\,\,\,\,\,\,{\text{Charge\ action,}}\\0\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,{\text{No\ charge\ or\ discharge\ action,}}\\  P_{{b_j}}^{\max,dis }\,\,\,\,\,\,\,\,\,\,\,\,\,\,\ {\text{Discharge\ action.}}\end{array} \right.\
% \end{equation}
% where $P_{{b_j}}^{\max,charge }$ and $P_{{b_j}}^{\max,dis }$ are maximum charge and discharge rate limits, respectively.

%------- Table DQN Hyperparameters

% \begin{table}[t]
%  \resizebox{\columnwidth}{!}{
% % \centering
%   {
%     \begin{tabular}{l|l|l}
%       \hline
%       \textbf{Hyperparameters} & \textbf{Value for $SPA$} & \textbf{Value for $PA_j$}\\
%       \hline
%       Batch size & 64 & 64 \\
%       Discount factor & ${\gamma}$=[0.95-0.99] & $\tilde{\gamma}_j$=[0.95-0.99] \\
%       Learning rate & $\alpha$=1e-3 & ${\tilde{\alpha}_j}$=1e-3 \\
%       Soft update interpolation & 1e-5 & 1e-5 \\
%       Hidden Layer-nodes & 1-[1000] & 2-[1000,1000] \\
%       Activation & Sigmoid & Sigmoid \\
%       Optimizer & Adam & Adam \\
%       \hline
%     \end{tabular}
%     }}
%     \caption{DQN Hyperparametrs Used in Our Simulations}
%     \label{tab:DQNhyperparameter}
%     \vspace{0.1in}
% \end{table}

\begin{table}[t]
\caption{DQN Hyperparameters and Simulation Parameters.}
\resizebox{0.7\columnwidth}{!}{
\centering
  {
    \begin{tabular}{l|l|l}
      \hline
      \textbf{Hyperparameters} & \textbf{Value for $SPA$} & \textbf{Value for $PA_j$}\\
      \hline
      Batch size & 64 & 64 \\
      Discount factor & ${\gamma}$=[0.95-0.99] & $\tilde{\gamma}_j$=[0.95-0.99] \\
      Learning rate & $\alpha$=1e-3 & ${\tilde{\alpha}_j}$=1e-3 \\
      Soft update interpolation & 1e-5 & 1e-5 \\
      Hidden Layer-nodes & 1-[1000] & 2-[1000,1000] \\
      Activation & Tanh & Tanh \\
      Optimizer & Adam & Adam \\
      \hline
      \hline
      \hline
      \textbf{Simulation Parameter} & \textbf{Description} & \textbf{Value}\\
      \hline
      $P_{PV_j}^{\max }$ & Max. PV Generation & [2-6] kW \\
      $P_{b_j}^{\text{max,charge} }/P_{b_j}^{\text{max,dis} }$ & Max. allowable charge/discharge & 2/-2.5 kW \\
      $P_{H_j}^{\max }$ & Max. allowable power injection & 10 kW \\
      ${SoC}_{b_j}^{\max }$ & Max. state of charge & $0.9 \times {C_{b_j}}$ \\
      ${SoC}_{b_j}^{\min }$ & Min. state of charge & $0.1 \times {C_{b_j}}$ \\
      $C_{b_j}$ & Energy storage capacity & [8-15] kWh \\
      ${\phi _j}(0)$ & Initial state of charge & [1-4] kWh \\
      $\rho _s$ & Sell price [before 11am, after 11am] & [0.05, 0.095] \$/kWh \\
      $\mathcal{A}_{SPA}$ & Buy price set for Agent-Based scenario & ${\{0.05,0.06,0.07,}$ \\ 
                  &                                    & ${0.08,0.09,0.1}\}$\$/kWh \\
      $\rho _b^t$ & Buy price for Conventional scenario & 0.06 \$/kWh \\
      $\left[ {P_{{G_1}}^{\min },P_{{G_1}}^{\max }} \right]$ & Limitation of base generation & [5, 45] kW  \\
      $\left[ {P_{{G_2}}^{\min },P_{{G_2}}^{\max }} \right]$ & Limitation of reserve generation & [0, 100] kW  \\
      $\left[ {\beta_1,\beta_2} \right]$ & Transmission loss coefficient of two generators & [0.0002, 0.0002] \\
      \hline
    \end{tabular}
    }}
 \label{tab:SimulationParam}
  \vspace{-0.1in}
\end{table}


\begin{figure}[t]
\centering
\includegraphics[scale=0.30, trim=0.2cm 0.2cm 0.2cm 0.2cm, clip]{figures/Price.png}
\vspace{-.2cm}
\caption{Retail prices for the last two days of the simulation.}
% . Sell price is the same for both Conventional and Agent-Based schemes. On the other hand, buy price is constant for the Conventional scheme, while  dynamically changing in the Agent-Based scenario (set by the SPA).}
\label{Price}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.24, trim=3cm 2cm 0.9cm 2cm, clip]{figures/5prosumers_profit.pdf}
\vspace{-0.1cm}
\caption{(a) Average daily bill comparison of the Conventional vs. Agent-Based schemes in a small-scale microgrid with 5 prosumers. (b) Performance comparison of the Conventional vs. Agent-Based scenarios in terms of grid profit and reserve unit utilization. }
\label{5prosumers_profit}
\vspace{-0.05in}
\end{figure}





% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.3, trim=1cm 0.01cm 1cm 0.5cm, clip]{figures/DailyBill_BarComparison.png}
% \vspace{-0.1cm}
% \caption{Average daily bill comparison of the Conventional vs. Agent-Based schemes in a small-scale microgrid with 5 prosumers.}
% \label{dailyBill_5prosumers}
% \vspace{-0.05in}
% \end{figure}



% \vspace{-0.2cm}
We compare the Agent-Based with the Conventional scheme through two scenarios: \textbf{(1)} A small-scale setting with 5 prosumers in which we demonstrate the agents' effectiveness in interacting with the energy marketplace environment, and improvements made to both SP and prosumers' economic benefits. \textbf{(2)} A medium-scale setting with 50 prosumers wherein we investigate the system's reliability and scalability by simulating a larger-scale microgrid. We implemented our DQN agents using Python3 with PyTorch 1.5.0.
% , and conducted the simulations on a desktop computer executing Windows 10 OS with an Intel Xeon processor (3 GHz) and 16 GB of RAM. 
All simulations were performed via episodic updating across 10,000 episodes, each of which represents a 24-h cycle. A cycle consists of 96 iterations (sampling time is 15 minutes).
\vspace{-0.1in}
% Sell price for both scenarios takes two constant values depending on the time of a day. Buy price is constant over the day in Conventional case, while it is dynamically determined by the service provider in Agent-Based scenario.
\subsection{Scenario I: Small-Scale Simulation with 5 Prosumers}
The first scenario studies the microgrid in Figure~\ref{fig:system-model} consisting of two generation facilities (a base plant and a spinning reserve) managed by one distribution SP, five prosumers, and one non-generational consumer. The DQN agents are implemented for the SP and the prosumers. The operational parameters of the five prosumers and the single consumer are tabulated in Table~\ref{tab:SimulationParam}. The utilized consumption and generation profiles for the prosumers mimic real-world  trends reported by California ISO \cite{CaliIso} to exemplify real-world operation.
%  Different levels of economic benefits for different prosumers is correlated with their PV power generation and consumption profiles, as we will explain in Figure~\ref{BattComparison}.  
\vspace{0.1in}
% \vspace{0.1in}
\subsubsection{\textbf{Macroscopic Evaluation of Prosumers and Grid Benefits}}
As reported in Table~\ref{tab:SimulationParam}, the sell price for both Conventional and Agent-Based scenarios takes two values depending on the time of a day. On the other hand, the buy price is constant during a day for the Conventional scenario, while in the Agent-Based scenario the buy price is dynamically determined by the SPA. Figure~\ref{Price} compares the dynamic pricing achieved by the Agent-Based approach vs. the fixed-pricing of the Conventional scheme. The results shown in Figure~\ref{5prosumers_profit} (a) compares the average daily bill of prosumers when utilizing the two approaches.  As pictured, the average daily bills have decreased by $22.1\%$, $8.2\%$, $10.9\%$, $48.8\%$, and $15.9\%$ for prosumer 1 to prosumer 5, respectively. Figure \ref{5prosumers_profit} (b) on the other hand, illustrates the moving average of SP profit and reserve generation consumption. According to these results, the Agent-Based approach is offering an $25.7\%$ increase in the SP profit, made possible by a $16\%$ reduction in reserve power consumption, compared to the conventional approach. This further demonstrates that the proposed Agent-Based approach is capable of providing a higher profit for the SP while offering greater economic benefit for the prosumers, warranting a win-win scenario for the grid and prosumers.  
% This demonstrates the effectiveness of the proposed Agent-Based approach to provide higher economic benefits to the prosumers.
% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.27, trim=0.2cm 0.2cm 0.3cm 0.2cm, clip]{figures/gridProfit_5prosumers.png}
% \vspace{-.3cm}
% \caption{Performance comparison of the Conventional vs. Agent-Based scenarios in terms of grid profit and reserve unit utilization. 
% % From the moving average results (over simulation episodes), the Agent-Based scheme improves economic benefits by reducing utilization of the costly reserve unit.
% }
% \label{gridProfit_5prosumers}
% \end{figure}
% \vspace{0.1in}
\subsubsection{\textbf{Microscopic Evaluation of  Prosumers' Behavior}}
Figure~\ref{BattComparison} illustrates the temporal profiles of several internal states of all five prosumers over the course of the last two simulated days for the Agent-Based and Conventional approaches. These graphs provide an intuitive interpretation of how each demand-side participators respond to the DR scheme in real-time. As pictured, using the Conventional method, the households' PV systems can charge their batteries only when their generation is more than consumption, while only being able to sell their excess generation when their batteries are fully charged. 
% By comparison with Figure~\ref{Price}, the Agent-Based method enables the prosumers to charge their batteries during the off-peak demand hours when the sell price is low, leading to reduced electricity bill, and selling the stored energy back to the grid when the sell price is high, for achieving further economic improvement and providing valuable peak shaving capacity to the grid during the peak demand hours.


\noindent \textbf{Observations on prosumers 1 and 2:} As demonstrated in Figure~\ref{BattComparison} (a) and (b), the generated power by prosumers 1 and 2 is less than their consumption (except for a very short period of time for prosumer 2). Therefore, throughout simulation of the Conventional approach, their batteries are never charging, denying them potential economic benefits otherwise possible by incorporating the energy storage system, and prohibiting them from participating in grid support during peak demand hours. On the other hand, using the Agent-Based approach, the prosumer batteries are charging during off-peak-low-price hours (i.e., beginning of the day), and prosumers are engaging in grid support during peak demand hours.  Although charging the battery at the beginning of the day incurs some cost for prosumers, it eventually provides higher economic benefits to them through selling the energy back to the grid at a higher price, while assisting with grid power balance during peak demand hours. 
In other words, the stored energy in prosumer 1 and 2 batteries is dispatched to the grid by properly incentivizing them to participate in DR.
 
 \begin{figure}[t]
\centering
\includegraphics[scale=0.39, trim=0.25cm 0.25cm 0.25cm 0.25cm, clip]{figures/Batt_Gen_ConComparison.png}
 \vspace{-0.3cm}
\caption{Generation and consumption profiles along with the State-of-Charge (SoC) for 5 prosumers.}
% Plots in (a) to (e) correspond to prosumer 1 through prosumer 5, respectively.}
\label{BattComparison}
 \vspace{-0.05cm}
\end{figure}


\noindent \textbf{Observations on prosumer 3:} According to consumption and generation profiles for prosumer 3 illustrated in Figure~\ref{BattComparison} (c), only a small amount of excess PV generation during a few hours is discernible. In this case, the results demonstrate that deploying the Agent-Based algorithm yields a higher SoC compared with the Conventional method. 
% is This implies that prosumer [3] will less support the grid during peak hours while 
% again in agent-based scenario the prosumer has been 
This is because the RL agent learns to charge the battery at the beginning of the day when the selling price by the grid is low, and to support the grid in the afternoon when the buy price is high. 
% Overall, the agent-based scheme provides more economic benefits for both grid and prosumers. 
% So, Leveraging the total capacity of the battery in agent-based scenario implies more grid supporting, and more grid supporting implies more economic benefits for both grid and prosumers.


\noindent \textbf{Observations on prosumers 4 and 5:} According to Figure~\ref{BattComparison} (d) and (e), these prosumers have excess PV generation during peak sun hours (e.g., around noon). The Conventional scheme fully charges the batteries of these prosumers during the peak sun hours, while the Agent-Based scheme charges the batteries starting from the beginning of the day when the sell price is low. As a result, these prosumers can sell their excess power during sun hours, rather than storing it, at even a higher price rate than the Conventional scheme could, after fully charging the batteries. 
% This results in further daily bill reduction compared with the Conventional scheme. 

% and.  This PA action provide will reduce prosumers' daily bill.


%Here both conventional and agent-based can support the grid perfectly during on-peak hours. Hence, there is no remarkable difference in economic benefits between these two scenarios. 


% \subsubsection{\textbf{Modeling and Incorporating Weather Data}}
% In the final experiment, 


\vspace{0.1in}
\subsubsection{\textbf{Effect of Battery Size}}
 %Next, we focus on the effect of prosumers' battery capacity on both daily bill and grid profit.
 Figure~\ref{Battsize} demonstrates the prosumers' daily bill reduction and grid daily profit achieved by increasing the size of prosumer batteries from $2$kWh to $25$kWh.  As pictured, the  daily bill for all five prosumers decreases as the battery capacities are increased. Similarly, the grid daily profit also increases by increasing the battery capacities. Nevertheless, the improvements start to level down as the battery capacities approach to around $15$kWh. Based on this observation, we use batteries with capacities in the range of $8$kWh to $15$kWh for all prosumers in the simulations. 
%  where the average daily payments and grid daily profit are reasonable.

Figure \ref{Trasmission_loss} demonstrates the impact of transmission losses on the total grid profit. In particular, the results show that as the value of transmission loss $\beta$ increases, the service provider profit decreases since it has to purchase more power to meet the total demand at any given time. 




% \begin{figure}
%     \begin{minipage}[c]{0.3\linewidth}
%         \centering
%         \includegraphics[scale=0.3, trim=0.5cm 0.25cm 0.5cm 1.5cm, clip]{figures/battSize-prosumers-1.png}
%         \caption{Effect of increasing battery capacity on the prosumers' average daily bill reduction in small-scale simulation.}
%     \end{minipage}\hfill
%      \begin{minipage}[c]{0.3\linewidth}
%         \centering
%         \includegraphics[scale=0.35, trim=0.5cm 0.05cm 0.5cm 0.5cm, clip]{figures/battSize-grid-1.png}
%         \caption{Effect of increasing battery capacity on the grid profit improvement in small-scale simulation. }
%     \end{minipage}
%     \label{fig:my_label}
% \end{figure}



\begin{figure}[t]
\centering
\includegraphics[scale=0.29, trim=1.2cm 0.2cm 0.5cm 2cm, clip]{figures/Batt_size.pdf}
\vspace{-.5cm}
\caption{(a) Effect of increasing battery capacity on the prosumers' average daily bill reduction in small-scale simulation. (b) Effect of increasing battery capacity on the grid profit improvement in small-scale simulation. 
% Average daily bill decreases as the battery capacity increases.
}
\label{Battsize}
\end{figure}




% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.3, trim=0.5cm 0.25cm 0.5cm 1.5cm, clip]{figures/battSize-prosumers-1.png}
% \vspace{-.3cm}
% \caption{Effect of increasing battery capacity on the prosumers' average daily bill reduction in small-scale simulation.
% % Average daily bill decreases as the battery capacity increases.
% }
% \label{Battsize-pr}
% \end{figure}


% \begin{figure}[t]
% \centering
% \vspace{-.3cm}
% \includegraphics[scale=0.3, trim=0.5cm 0.05cm 0.5cm 0.5cm, clip]{figures/battSize-grid-1.png}
% \vspace{-.1cm}
% \caption{Effect of increasing battery capacity on the grid profit improvement in small-scale simulation. 
% % Grid profit increases as the battery capacity increases.
% }
% \label{Battsize-grid}
% \end{figure}


\vspace{-.20cm}
% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.35, trim=0.5cm 0.5cm 0.5cm 0.5cm, clip]{figs/50Prosumers.pdf}
% \vspace{-.20cm}
% \caption{Medium scale microgrid in presence of $N_p$ prosumers and $N_c$ consumers where $N_p=50$ and $N_c=40$.  }
% \label{50prosumers}
% \end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.135, trim=6cm 0.3cm 7cm 0.5cm, clip]{figs/consumerProfile.png}
% \vspace{-.1cm}
% \caption{Total consumption profile for $N_c = 40$ non-generational consumers in one day.}
% \label{ConsumerProfile}
% \end{figure}

\subsection{Scenario II: Medium Scale Simulation with 50 Prosumers}

\begin{figure}[t]
\centering
\vspace{-.3cm}
\includegraphics[scale=0.31, trim=1cm 0.25cm 0.5cm 1cm, clip]{figures/Transmission_loss_comparison.png}
% \vspace{-.2cm}
\caption{Impact of transmission losses on total grid profit.
% Average daily bill decreases as the battery capacity increases.
}
\label{Trasmission_loss}
\end{figure}


The second scenario studies a medium scale microgrid with $50$ prosumers and $N_c = 40$ non-generational consumers.
% as shown in Figure~\ref{50prosumers}. 
% The total demand profile for the $40$ consumers during a 24-hour period is 
% provided in \cite{9449714}.
% shown in Figure~\ref{ConsumerProfile}. 
In this scenario, the proposed method's scalability is the main criteria under investigation.
% We also compared the average daily electricity charges for prosumers in agent-based scenario with conventional scenario in Fig.~\ref{50Prosumers_profit}. 
The average daily electricity bills for 50 prosumers each with a distinct consumption profile, while using Conventional and Agent-Based approaches are illustrated in Figure~\ref{50Prosumers_profit}(a). According to this figure, the average daily bill is reduced for all 50 prosumers in the Agent-Based scenario. Figure~\ref{50Prosumers_profit}(b) represents the probability distribution function of the average daily bill for 50 prosumer data points. This figure illustrates an average bill of $\$1.96$ for Conventional method, vs. $\$1.74$ for Agent-Based method, amounting to around $12\%$ bill reduction for a 24 hour billing cycle. 

% \begin{figure*}[h]
% \centering
% \includegraphics[scale=0.4, trim=0.5cm 0.08cm 0.5cm 0.5cm, clip]{figs/probability.pdf}
% \vspace{-.3cm}
% \caption{Average daily bill comparison for Conventional vs. Agent-Based scenarios in 50 prosumers study (a) average daily bill comparison for 50 prosumers (b) Distribution of average daily bills for 50 prosumers. These results confirm that the Agent-Based scheme is scalable and provides economic benefits to all 50 prosumers.}
% \label{50Prosumers_profit}
% \end{figure*}
% \begin{figure}[t]
% % \centering
% \includegraphics[scale=0.28, trim=2.1cm 0.9cm 1.5cm 1.5cm, clip]{figures/probability-vertical.pdf}
% \vspace{-.08cm}
% \caption{Performance of the Conventional vs. Agent-Based scenarios in the medium scale microgrid with 50 prosumers. (a)~Average daily bills of prosumers; (b) Distribution of average daily bills. 
% % These results confirm that the Agent-Based scheme is scalable and provides economic benefits to all 50 prosumers.
% }
% \label{DailyBillPr}
% \vspace{-0.05in}
% \end{figure}
% \begin{figure}[h]
% \centering
% \vspace{-.2cm}
% \includegraphics[scale=0.26, trim=0.3cm 0.1cm 0.2cm 0.1cm, clip]{figures/gridProfit_50prosumers.png}
% \vspace{-.3cm}
% \caption{Performance comparison of the Conventional vs. Agent-Based scenarios in terms of grid profit and reserve power consumption with $50$ prosumers. 
% % The  Agent-Based  scheme  improves  economic benefits  by  reducing  utilization of the costly reserve unit.
% }
% \label{GridProfit_50Pr}
% % \vspace{-0.1in}
% \end{figure}
Figure~\ref{50Prosumers_profit} (c) compares the accumulative grid profit and reserve power utilization of the Conventional and Agent-Based scenarios in our medium scale microgrid. As pictured, the Agent-Based method provides around $4.3\%$ higher profit over a 24-hour period. This improvement is due to the fact that the SPA and PAs learn how to dispatch the batteries' power to rely on the prosumers' PV generation, rather than using the costly reserve power. 
Moreover, properly incentivizing the prosumers to dispatch their stored energy has a positive impact on shaving the peak load demand of the grid, as compared in Figure~\ref{AveragePnet} over a 24-hour period. 
% This figure illustrates the total demand profile of the simulated microgrid with a base load generation capacity of $390$kW.  
As pictured, the Agent-Based approach shifts the demand at the peak hours between 18pm to 24pm to early morning hours before 6am.  
% This peak demand is usually met with very costly peaking power plants in conventional systems.  Therefore, the Agent-Based approach can greatly lesson the need for using utilizing these costly peaking power plants.      
\begin{figure}[t]
% \centering
\includegraphics[scale=0.205, trim=2.5cm 0.7cm 0.05cm 2.2cm, clip]{figures/50prosumer_profit.pdf}

\caption{Performance of the Conventional vs. Agent-Based scenarios in the medium scale microgrid with 50 prosumers. (a) Average daily bills of prosumers; (b) Distribution of average daily bills; (c) Performance comparison of the Conventional vs. Agent-Based scenarios in terms of grid profit and reserve power consumption with $50$ prosumers.
}
\label{50Prosumers_profit}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[scale=0.35, trim=0.5cm 0.1cm 0.5cm 1cm, clip]{figures/AveragePnet.png}
\caption{Average net power comparison for the Conventional vs. Agent-Based scenarios during a 24-hour period. 
% The Agent-Based scheme reduces the maximum net demand during peak hours.
}
\label{AveragePnet}
\end{figure}


==> ACM Journal paper/chapters/7.Conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we propose a Deep Reinforcement Learning (DRL) framework for energy management and demand response in prosumer dominated microgrids. The service provider DRL agent dynamically changes the electricity buy price and determines the direction and amount of power flow according to the household's load demand. Further, the prosumers DRL agent controls the battery charge and discharge rate and amount of power injection into the grid. These DRL agents collectively provide a dynamic decision-making framework. 
% To show the effectiveness and robustness of the proposed algorithm, numerical results has been simulated for two, small-scale and medium scale scenarios.  
Our  simulation results demonstrate that the proposed framework provides higher economic benefits for both power grid and prosumers. Specifically, properly incentivizing prosumers through dynamic pricing and leveraging the capacity of distributed battery resources result in: (i) reduced average daily bills for prosumers, (ii) enhanced profits for the grid by decreasing the reserve generation power demand, and (iii) reduced net power demands during peak hours. 
The proposed framework can be extended by including other external observations such as weather conditions, or investigating the performance of DRL agents under peer-to-peer energy sharing  across prosumers.  




% The result of this paper can be extended in several directions. First, in this paper, we did not study the system's reliability under the influence of weather condition changing. We are planning to discuss this impact in our future work. Second, in our work, we assumed that the service provider is dealing with two generation facilities as base and spinning reserve. However, in practice, there are several kinds of generation facilities that make the economic benefit of service provider more challenging. This is another interesting future direction of this work. Third, peer-to-peer energy sharing between prosumers provides a more challenging retail market, which leads to extensive research interest. The proposed RL solution in this paper grants the opportunity to a less complicated solution in considering these kinds of challenges.


% These benefits are achieved We show that by the agents learning ability and without any prior knowledge (1) prosumers with different consumption and generation patterns can  to reduce their daily bill, (2) grid increases its profit while reducing the reserve generation power demand, (3) Providing a win-win scenario will encourage prosumers to participate in grid support program (4) And as a result, reduce the peak of net power demand and flatten the net demand curve to some extent. 

==> ACM Journal paper/chapters/RelatedWork_new.tex <==
\section{Related work}
\label{sec:related_work}

The interaction between service provider and end-users have been investigated in many prior works. Recently, there has been growing interests in adopting RL to address the concerns of this interaction. These attempts can be categorized as follows:

\textbf{Prior Works Focused on Service Provider}: 
A multitude of prior works use RL in the context of power systems, mainly to address service provider concerns. 
% For instance, constrained energy trading between end-users was investigated in~\cite{wang2016reinforcement}.
For example, a hierarchical electricity market with bidding and pricing over wholesale and retailer using DRL was proposed 
in~\cite{xu2019deep}. In ~\cite{liang2020agent}, a Deep Deterministic Policy Gradient (DDPG) algorithm was used to solve the bidding problem of several generation companies. Moreover, RL has been widely employed for energy management optimization~\cite{foruzan2018reinforcement, dridi2021novel}. In~\cite{foruzan2018reinforcement}, the authors proposed a multi-agent distributed energy management using Q-learning framework with time-of-use pricing for a microgrid energy market with a centralized battery pack and renewable generation. The authors in \cite{dridi2021novel} designed a novel RL method that uses classical recurrent neural networks instead of SAR (State-Action-Reward) method to solve the microgrid energy management in the Industrial Internet of Things (IIoT).
In contrast to these works, we propose a dynamic pricing scheme with DQN at the service provider side, combined with distributed battery and PV installations at the demand side. 



\textbf{Prior Works Focused on End-users}: 
The authors in \cite{wang2020deep} developed a DDQN-based load scheduling
algorithm with a time-of-use scheme to reduce the peak load demand and the operation cost for the distribution system, however without considering prosumers. In~\cite{chung2020distributed}, the interaction between households and the service provider was modeled to jointly solve the energy scheduling consumption and preserving privacy for the households by using policy gradient RL method.
Furthermore, \cite{9281326} developed a home energy management system (HEMS) using Actor-Critic technique based on adaptive dynamic programming.
Likewise, in \cite{7401112}, an energy management DR using Q-learning adjusts 
the consumption plan for thermostatically controlled loads. 
Along the same lines, \cite{xu2020multi} proposed a framework for home energy management based on multi-agent Q-learning to minimize the electricity bill as well as DR-induced dissatisfaction costs for end-users. 
Their method considered proliferation of rooftop PV systems, but did not consider home energy storage systems. Moreover, the works in \cite{sun2020continuous,yang2019large}, focused on reducing the high peak load in large-scale HEM using Entropy-based multi-agent deep reinforcement learning, and the work in \cite{ye2020model} applied prioritized DDPG in multi-carrier energy system to solve the real-time energy management problem.
It is also worth noting that these works \cite{wang2020deep,chung2020distributed,9281326,7401112,xu2020multi,sun2020continuous,yang2019large} do not consider the grid side and only propose optimization algorithms for end-users.

\textbf{Prior Works Focused on Both Service Provider and End-users}: Other research works have addressed the interactions between retailer/SP and end-users. 
For example, \cite{samadi2014real} investigated a gradient-based method to minimize the 
aggregate load demand by assuming the presence of consumption scheduling devices on the users side.   
Furthermore, works such as \cite{jia2016dynamic, yu2018incentive,8490840} leveraged the Stackelberg game
to model and maximize 
the retailer profit and minimize the payment bill of its customers. 
The authors included renewable energy generation on the retailer side, which is different from our model 
with distributed PV installations across prosumers. 
The studies in \cite{dehghanpour2016agent} and \cite{lu2019incentive} proposed a hierarchical agent-based framework 
% for implementing a price-based DR program 
to maximize both retailer and customers profits. %The study reported in \cite{dehghanpour2016agent} used Q-learning for decision making problem in lower level side (end-user) and linear and ANN model model for upper level side (retailer) was used and their model can be used for load shaving as well.  
A Q-learning DR is proposed in \cite{DynamicPrice} for the energy consumption scheduling problem that can work without prior information and leads to reduced system costs. Also, in \cite{11Dynamic} both service provider profit and consumers' cost are considered to find the optimal retail price. However, unlike our effort, the works presented in \cite{dehghanpour2016agent,lu2019incentive,DynamicPrice,11Dynamic} only consider regular electricity consumers, rather than prosumers with generation and storage capabilities. 
In contrast to these efforts, we model a microgrid that consists of both consumers and prosumers that are equipped with battery storage. As a result, the proposed multi-agent DRL framework achieves DR with dynamic pricing and distributed energy management for a microgrid with large-scale rooftop PV panels and energy storage system.
Table~\ref{tab:relatedwork} compares our work 
with the previous related works. 

\begin{table}
%  	\centering
 		\caption{Taxonomy of Related Work on Management of Distributed Energy Resources. (\Checkmark : Considered, ---: Not Considered ) }
 	\resizebox{\columnwidth}{!}{
  	\begin{tabular}{|l|c|c|c|c|c|}
  	\hline
  	\textbf{Reference} & \textbf{Energy management } & \textbf{Retailer/end-user} & \textbf{Renewable penetration}
  	& \textbf{Energy storage} & \textbf{RL} \\
  	 & \textbf{DR} & \textbf{profit optimization}  & \textbf{consideration} & \textbf{consideration}  & \textbf{algorithm}\\
  	 \hline
  	\cite{dehghanpour2016agent},\cite{DynamicPrice},\cite{11Dynamic} & \Checkmark & \Checkmark & --- & --- &\Checkmark \\
  	\hline
  	\cite{yu2018incentive},\cite{8490840},\cite{chung2020distributed},\cite{lu2019incentive}& \Checkmark & \Checkmark  & --- & --- & ---\\ 
  	\cite{xu2020multi} & ---& \Checkmark& \Checkmark  & --- & \Checkmark \\
  	\hline
  	\cite{sun2020continuous}, \cite{yang2019large} & --- & \Checkmark & --- & --- & \Checkmark\\
  	\hline
  	\cite{jia2016dynamic} & \Checkmark & --- & --- & \Checkmark & \Checkmark \\
  	\hline
  	Our proposed framework & \Checkmark &  \Checkmark & \Checkmark & \Checkmark  & \Checkmark \\ 
  	\hline
 	\end{tabular}}
 	\vspace{-0.1in}
 	\label{tab:relatedwork}
 \end{table}


==> ACM Journal paper/chapters/intro_new.tex <==
\section{Introduction}
Recent proliferation in renewable energy sources (RESs) and distributed energy resources (DERs) along with the advances in information and communication technologies (ICT) has  facilitated a paradigm  shift  from  the traditional 
power consumers to the more resourceful energy \emph{prosumers}. 
A prosumer is an active end-user with the ability to consume and produce energy~\cite{5759167}. The number of prosumers is increasing as more households are proceeding to install  solar photovoltaic (PV) rooftop panels and energy storage system (ESS)~\cite{ 7820171}. The premise of such a distributed network of energy resources is to provide economic and ancillary benefits 
to both prosumers and power grid service provider (SP)~\cite{khoshjahan2021impacts}. The interaction between the prosumers and SP has been investigated in several prior studies. Many works utilize model-based control paradigms, such as model predictive control (MPC)~\cite{gan2020data}, mixed-integer linear programming (MILP)~\cite{7114268}, dynamic and stochastic programming~\cite{farzaneh2019robust}, and alternating direction method of multiplier (ADMM)~\cite{7501891}. 
One key step for applying these techniques is to establish an accurate model that captures the dynamics of the microgrid and the interactions between various components with all the operational constraints.



% achieve cost reduction or other interest.
% The ultimatelty goaenable a beneficial interaction, and win-win scenario between the SP and the prosumers.

 The massive deployment of DERs and RESs dramatically increases the complexity and uncertainty of the system due to the more complex cross-area power balancing between SP and prosumers. This makes the accurate system model hard to obtain. The model-based nature of the aforementioned methods also exhibits limited generalization capabilities~\cite{dorokhova2021deep}. Difficulties in handling nonlinear behavior, volatile renewable generations, and heterogeneity of the end-users represent other major shortcomings of these methods. To overcome these challenges, model-free Reinforcement Learning (RL) techniques are proven beneficial for demand-side energy management since they do not require an explicit model of the environment. In general, RL frameworks are emerging as the pre-eminent tool for sequential decision-making problems within unknown environments. Similar to many other scientific and engineering domains, the RL-based solutions are receiving more attention from the power system society. For instance, voltage and frequency control \cite{wang2021multi}, market bidding \cite{pedasingu2020bidding}, microgrid energy management \cite{samadi2020decentralized}, and demand response (DR) \cite{vazquez2019reinforcement} are just a few examples of power-related problems that can be solved using RL.
%  In addition, it is more challenging for the SP to estimate the impact of its online pricing on customers' future behavior while considering the long-term performance of the microgrid.
%  Overall, the conventional model-based optimization techniques have to compute all the possible solutions on small-time horizons that results in high computational complexities and inefficiency for online use.

% However, it should be noted that high penetrations of RESs and DERs may cause instability in the smart grid due to output voltage volatility as well as limited controllability and predictability. To mitigate these issues, DR programs provide the gird more flexibility. The purpose of DR is to incentive the prosumers to actively participate in a program, and contribute to the optimal energy distribution in electricity retail market. 

 


In this paper, and to bridge the gap between the power system and RL communities, we investigate the mutual interplay between participants and the different tasks in a residential microgrid. We propose a framework based on Deep Reinforcement Learning (DRL) for both SP and prosumers to enable dynamic decision-making.  A service provider agent (SPA) is deployed for solving the distributed energy management (DEM) problem in the microgrid by dynamically determining  the electricity buy price as a control parameter for optimization of the energy management across distributed prosumers. For instance, a higher electricity buy price during peak hours (e.g., evening hours) incentivizes the prosumers with surplus energy to discharge their battery. As a result, the prosumer receives economic benefit in terms of electricity bill reduction. This process is called Demand Response (DR).  The purpose of DR is to encourage the prosumers to actively participate in a program and contribute to the optimal energy distribution in the electricity retail market.  Moreover, buying electricity from distributed prosumers would enable the power grid service provider to support higher demands during peak hours. In our envisioned system model, the prosumer agent (PA) solves the prosumer energy management problem by determining the charge/discharge of the battery installation. Thus, each prosumer independently  maximizes its own profit. 

In summary, our main contributions are as follows:
\vspace{-0.15cm}
\begin{itemize}
 \item We formally define the interaction between SP and the prosumers as a Markov Decision Process (MDP), and develop a multi-agent DRL framework that interweaves the real-time energy management over the microgrid with the prosumer side real-time DR, using demand-dependent dynamic pricing for incentivizing prosumers' participation in DR.
  \item We show that the proposed DRL framework enables the service provider to leverage energy storage as dispatchable assets, while incentivizing the prosumers to actively participate in the program to support the grid activities.
 \item Our numerical results based on Deep Q-Network (DQN) demonstrate that the proposed framework reduces the average daily bill for prosumers, while at the same time it provides higher profits for the grid service provider (SP) by leveraging distributed energy resources instead of tapping into traditional reserve generation facilities with higher costs.  
\end{itemize}
The remainder of this paper is organized as follows. Section~\ref{sec:related_work} 
covers related work, followed by the system model and problem formulation in Section~\ref{sec:model}. 
Next, Section~\ref{sec:RLmodel} formulates the DRL framework and Section~\ref{sec:result} presents numerical results. Finally, Section \ref{sec:conclusion} concludes the paper. 



% %############################################################

% Intermittent output of renewable energy resources (RES) has provided more challenges to retail electricity market due to more complex cross-area power balancing between supply and demand.

% %############################################################


==> chapters/2.Introduction.tex <==

\section{Introduction}
Advances in renewable energy generation and their availability as local 
energy resources in power systems facilitate a paradigm  shift  from  the traditional 
power consumers to the more resourceful energy \emph{prosumers}. 
A prosumer is an end-user with the ability to consume and produce energy ~\cite{5759167}. 
The number of prosumers is increasing as more households are proceeding to install 
Distributed Energy Resources (DERs), such as solar photovoltaic (PV) panels~\cite{ 7820171}.   
The premise of DERs is to provide economic and ancillary benefits 
to both prosumers and power grid service provider (SP). However, achieving the full potential of 
distributed household PV systems is challenging due to two main factors. 
\textbf{(1)} Currently, households with PV systems can only sell their excess energy during the 
daylight hours when the price of electricity is low.
\textbf{(2)} Current popular net-metering compensation schemes leave prosumers with limited 
economic benefits and little incentive to engage in grid support applications~\cite{corbett2018toward}.
As a result, existing models for integration of DERs into the grid create a non-profitable 
situation for both prosumers and SP~\cite{chakraborty2018analysis}. 
To mitigate these issues, integrating energy storage devices with DERs provides 
more flexibility for prosumers to participate in \emph{Demand Response} (DR)  programs~\cite{7063260}. Additionally, SP will accomplish higher profit through implementing distributed energy management (DEM) for residential DERs with bidirectional power flow. Therefore, a dynamic decision-making framework that combines DR and DEM can provide a win-win scenario for both prosumer and SP.

There are several works that utilize model-based control paradigms for microgrid and demand-side energy management problems, such as model predictive control (MPC)~\cite{gan2020data}, mixed-integer linear programming (MILP)~\cite{7114268}, dynamic and stochastic programming~\cite{farzaneh2019robust}, and alternating direction method of multiplier (ADMM)~\cite{7501891}. 
One key step for applying these techniques is to establish an accurate model that captures the dynamics of the microgrid and the interactions between various components with all the operational constraints. The model-based nature of these methods also exhibits limited generalization capabilities~\cite{dorokhova2021deep}.  Difficulties in handling nonlinear behavior, volatile renewable generations, and heterogeneity of the end-users represent other major shortcomings of these methods. In addition, it is more challenging for the SP to estimate the impact of its online pricing on customers' future behavior while considering the long-term performance of the microgrid. Overall, the conventional optimization techniques have to compute all the possible solutions on small-time horizons that results in high computational complexities and inefficiency for online use.

To overcome the aforementioned challenges, model-free Reinforcement Learning (RL) techniques are proven beneficial for demand-side energy management problems since they do not require an explicit model of the environment, which is challenging to acquire in practice. In this paper, we investigate the mutual interplay between participants and the different tasks in a residential microgrid. We propose a framework based on Deep Reinforcement Learning (DRL) for both SP and prosumers to enable dynamic decision-making.  A service provider agent (SPA) is deployed for solving the distributed energy management (DEM) problem in the microgrid by dynamically determining  the electricity buy price as a control parameter for optimization of the energy distribution. On the other side, the presence of prosumers provides a large-scale integration of DER schemes with different owners that tend to maximize their own profit without considering the other owners and the SPA performance. Here, the prosumer agent (PA) solves the prosumer energy management problem by determining the charge/discharge of the prosumer's battery installation. In summary, our main contributions are as follows:
% \vspace{-0.025in}
\begin{itemize}
 \item We develop a multi-agent DRL framework that interweaves the real-time energy management over the microgrid with the prosumer side real-time DR, using demand-dependent dynamic pricing for incentivizing prosumers' participation in DR.
  \item We show that the proposed DRL framework enables the service provider to leverage energy storages as dispatchable assets, while incentivizing the prosumers to actively participate in the program to support the grid activities.
 \item Our numerical results demonstrate that the proposed framework reduces the average daily bill for prosumers, while at the same time it provides higher profits for the grid service provider (SP) by leveraging distributed energy resources instead of tapping into traditional reserve generation facilities. 
\end{itemize}
The remainder of this paper is organized as follows. Section~\ref{sec:related_work} 
covers related work, followed by the system model and problem formulation in Section~\ref{sec:model}. 
Next, Section~\ref{sec:RLmodel} formulates the DRL framework, while Section ~\ref{sec:result} presents numerical results. Finally, Section \ref{sec:conclusion} concludes the paper. 

==> chapters/3.Relatedwork.tex <==
\section{Related work}
\label{sec:related_work}

% \mycomment{YD: I think the related work section could use some organization and precision by grouping similar works together}
% \mycomment{Alex: It may be good to go back to using in-line subtitles to label the different kinds of related works. It may be easier to follow and you can remove quite a few connection words such as furthermore, moreover, etc.}
A multitude of prior works use RL in the context of power systems, mainly to locate optimal pricing. 
For instance, 
% a bidding strategy for an agent-based local microgrid was proposed in~\cite{7300459} 
% where each agent is responsible for trading electricity with other agents and maximizing their profit 
% in a local energy market with no grid connection. 
constrained energy trading between end-users was investigated in~\cite{wang2016reinforcement}.
% where adaptive RL was used to converge the bidding problem between participants. 
A hierarchical electricity 
market with bidding over wholesale and retail using RL was proposed 
in~\cite{xu2019deep}, while in~\cite{liang2020agent} a DDPG algorithm was used to solve the bidding problem 
of several generation companies. Moreover, RL have been widely employed for energy management optimization~\cite{foruzan2018reinforcement, 123456}. In~\cite{foruzan2018reinforcement}, the authors proposed a multi-agent distributed energy management framework with time-of-use pricing for a microgrid energy market with a centralized battery pack and renewable generation. 
% They used a Q-table algorithm with time-of-use pricing for solving the distribution optimization problem. 
In this work, we propose a dynamic pricing scheme with DQN for distributed battery and PV setup penetration. In~\cite{123456}, RL methods were utilized to manage the energy in a multi-microgrid system. 










% A multitude of prior works use RL in the context of power systems mainly to locate optimal pricing. 
% For instance, a bidding strategy for an agent-based local microgrid was proposed in~\cite{7300459} 
% where each agent is responsible for trading electricity with other agents and maximizing their profit 
% in a local energy market with no grid connection. 
% On the other hand, several works used RL by focusing on the single objective of 
% minimizing the cost of generation~\cite{8306311 ,9255238,dai2019distributed}. 
% In ~\cite{8306311}, Liu \emph{et al.} proposed a cooperative reinforcement learning approach 
% to solve the ED problem in microgrids with distributed generation resources and energy storage systems 
% with the goal of optimizing the cost of microgrid operations as well as satisfying the power constraints. 
% %which is not considered prosumers. 
% % In \cite{9255238},  the ED problem has been solved for a simple power system model. 
% Dai \emph{et al.}~\cite{dai2019distributed} also deployed reinforcement learning to solve the dynamic 
% economic dispatch problem to find the optimal output of each unit. 
% A multi-agent RL method with the objective of minimizing both fuel cost and emission in the 
% traditional power system model without renewable resources is proposed in~\cite{mannion2016dynamic}. 
% In \cite{8957677}, a deep reinforcement learning algorithm is proposed to obtain economic dispatch 
% in virtual power plants that are part of distributed energy resources, however, 
% the objective was still minimizing the operating cost of distributed generation (DG) resources 
% including photovoltaic and wind turbine. Although these prior efforts use RL in power systems 
% to locate optimal pricing, they do not include the newly arising entity covered in our work, 
% specifically the prosumers. 

Other research projects have addressed the interactions between retailer/SP and end-users. 
For example, \cite{samadi2014real} investigated a gradient-based method to minimize the 
aggregate load demand by assuming the presence of consumption scheduling devices on the users' side.   
Furthermore, works such as \cite{jia2016dynamic, yu2018incentive,8490840} leveraged the Stackelberg game
% . 
% Specifically, \cite{jia2016dynamic} used a Stackelberg game 
to model and maximize 
the retailer profit and minimize the payment bill of its customers. 
The authors included renewable energy generation on the retailer side, which is different from our model 
with distributed PV installations across prosumers. 

% \emph{Related Work on Demand Response:} 
% The conventional time-based DR approaches, such as the real-time pricing methods, mostly focus on altering the preferred electricity consumption pattern of the consumer, e.g. 
% by 
% % changing the temperature set point on air conditioning systems or 
% delaying the use of major appliances, in order to shift their load to off-peak hours.  However, these approaches lead to the dissatisfaction of consumers and therefore they have not been widely adopted thus far \cite{pinson2014benefits , haider2016review}. In contrast, our proposed prosumer side DR algorithm does not alter the consumption pattern of the households (no disutility).  Rather, it achieves cost savings by altering the households' power demand pattern, using the flexibility provided by energy storage coupled with PV generation.

% \cite{chen2013mpc} proposed a  model predictive control (MPC) based for appliance scheduling scheme of home energy management system to minimize consumer energy cost which does not consider the grid side. 


%Similarly, Stackelberg game was adopted in \cite{yu2018incentive} to model and analyze decision making components across the  service provider, and conventional and industrial consumers, i.e., no prosumer was considered.

%In \cite{zhang2017robust}, the overall economic benefits of operators and customers are optimized with price-based demand response. However, no energy storage and renewable energy are included in this model. 
% A two-stage robust optimization (TSRO) and column-and-constraint generation (C$\&$CG) algorithm is employed to ensure the optimization results are robust against all uncertainties however there is no energy storage and renewable energy in the model. 
On a different note, \cite{wang2020deep} developed a DRL-based load scheduling 
algorithm with a time-of-use scheme to reduce the peak load demand and the operation cost for the 
distribution system, however without considering prosumers. In~\cite{chung2020distributed} the interaction between households and the aggregator was modeled to jointly solve the energy scheduling consumption and preserving privacy for the households by using policy gradient RL method.
Furthermore, \cite{9281326} developed a home energy management system (HEMS) using Actor-Critic technique based on adaptive dynamic programming.
% that focuses on the consumer's dissatisfaction in a conventional setup and 
% without any renewable resources. 
Likewise, in \cite{7401112}, an energy management DR using RL adjusts 
the consumption plan for thermostatically controlled loads. 
%In \cite{7792709}, batch reinforcement learning technique is used for water heater consumption control using auto-encoder network to reduce the dimensionality of the state-space.
% The authors in \cite{8928284} investigated a DR problem for household heating system and electric water heater by applying a combination of two neural networks (convolutional and LSTM) and RL, and they did not consider renewable resources and energy storage for consumers.
Along the same lines, \cite{xu2020multi} proposed a framework for home energy management based 
on RL to minimize the electricity bill as well as DR-induced dissatisfaction costs for end-users. 
Their method considered proliferation of rooftop PV systems but did not consider
home energy storage systems. Moreover, \cite{bahrami2020deep} proposed a 
DRL approach to reduce peak load and household cost by load scheduling in an IEEE 33-bus test feeder with 
32 consumers. They demonstrated 33$\%$ reduction in peak load and 13$\%$ reduction in households' 
daily cost, without considering any storage system.
It is also worth noting that these works \cite{wang2020deep,7042790,7401112, 8928284,xu2020multi,bahrami2020deep} do not consider the grid side and only propose optimization algorithms for end-users.
% \mycomment{AB: How is our work different from these works?}

% Energy storage system has not been considered in none of the aforementioned researches which in our latest work \cite{Ghasemi} has shown that can be an effective parameter to improve the system efficiency in terms of reducing costs.
%Although some of the aforementioned works have considered the penetration of PV generations, none of them considered battery capabilities.
% \vspace{-0.1in}


% Both retailer and end-users profits maximization  has been studied in \cite{dehghanpour2016agent,lu2019incentive,DynamicPrice,11Dynamic}. 
The studies in \cite{dehghanpour2016agent} and \cite{lu2019incentive} proposed a hierarchical agent-based framework 
% for implementing a price-based DR program 
to maximize both retailer and customers profits. %The study reported in \cite{dehghanpour2016agent} used Q-learning for decision making problem in lower level side (end-user) and linear and ANN model model for upper level side (retailer) was used and their model can be used for load shaving as well.  
An RL-based DR is proposed in \cite{DynamicPrice} for the energy consumption scheduling problem that can work without prior information and leads to reduced system costs. Also, in \cite{11Dynamic} both service provider profit and consumers' cost are considered to find the optimal retail price. However, unlike our effort, the works presented in \cite{dehghanpour2016agent,lu2019incentive,DynamicPrice,11Dynamic} only consider regular electricity consumers, rather than prosumers with generation and storage capabilities. 
In contrast to these efforts, we model a microgrid that consists of both consumers and prosumers that are equipped with battery storage. As a result, the proposed multi-agent DRL framework achieves DR with dynamic pricing and distributed energy management for a microgrid with large-scale rooftop PV panels and energy storage system.
Table~\ref{tab:relatedwork} compares our work 
with the previous related work. 


\begin{table}
%  	\centering
 		\caption{Taxonomy of Related Work on Management of Distributed Energy Resources. (\Checkmark : Considered, ---: Not Considered ) }
 	\resizebox{\columnwidth}{!}{
  	\begin{tabular}{@{}lccccc@{}}\toprule
  	\textbf{Reference} & \textbf{Energy management } & \textbf{Retailer/end-user} & \textbf{Renewable penetration}
  	& \textbf{Energy storage} & \textbf{RL} \\
  	 & \textbf{DR} & \textbf{profit optimization}  & \textbf{consideration} & \textbf{consideration}  & \textbf{algorithm}\\
  	\midrule \cite{dehghanpour2016agent},\cite{DynamicPrice},\cite{11Dynamic} & \Checkmark & \Checkmark & --- & --- &\Checkmark \\
  	\cite{yu2018incentive},\cite{8490840},\cite{chung2020distributed},\cite{lu2019incentive}& \Checkmark & \Checkmark  & --- & --- & ---\\ 
  	\cite{xu2020multi} & ---& \Checkmark& \Checkmark  & --- & \Checkmark \\
  	\cite{wang2020deep}, \cite{bahrami2020deep} & --- & \Checkmark & --- & --- & --- \\
  	\cite{jia2016dynamic} & \Checkmark & --- & --- & \Checkmark & \Checkmark \\
  	Our proposed framework & \Checkmark &  \Checkmark & \Checkmark & \Checkmark  & \Checkmark \\ 
 	\bottomrule
 	\end{tabular}
 	}
 	\vspace{-0.1in}
 	\label{tab:relatedwork}
 \end{table}

